A Neural Approach to Spatio-Temporal Data Release with User-Level Differential Privacy

Several companies (e.g., Meta, Google) have initiated "data-for-good" projects where aggregate location data are first sanitized and released publicly, which is useful to many applications in transportation, public health (e.g., COVID-19 spread) and urban planning. Differential privacy (DP) is the protection model of choice to ensure the privacy of the individuals who generated the raw location data. However, current solutions fail to preserve data utility when each individual contributes multiple location reports (i.e., under user-level privacy). To offset this limitation, public releases by Meta and Google use high privacy budgets (e.g., $\epsilon$=10-100), resulting in poor privacy. We propose a novel approach to release spatio-temporal data privately and accurately. We employ the pattern recognition power of neural networks, specifically variational auto-encoders (VAE), to reduce the noise introduced by DP mechanisms such that accuracy is increased, while the privacy requirement is still satisfied. Our extensive experimental evaluation on real datasets shows the clear superiority of our approach compared to benchmarks.

==> Spatiotemporal data release (1)/bck.tex <==
%\subsection{Differential Privacy} \label{subsec:dp}
\subsection {Differential Privacy}
%$\varepsilon$-differential privacy~\cite{dwork2014algorithmic} provides a rigorous framework with formal protection guarantees. 
{Given {\em privacy budget} $\varepsilon \in (0, +\infty)$}, a mechanism $\mathscr{M}$ satisfies $\varepsilon$-differential privacy~\cite{dwork2014algorithmic} iff for any {\em sibling} datasets $D$ and $D^\prime$  differing in a single tuple, and for all $E \subseteq$ Range($\mathscr{M}$)%\vspace*{-4pt}
\begin{equation}
\vspace*{-4pt}
\text{Pr}[\mathscr{M}(D) \in E] \leq e^\varepsilon \text{Pr}[\mathscr{M}(D^\prime) \in E]
\end{equation}

%{$\text{Pr}[\mathscr{M}(D) \in E]$ denotes the probability of mechanism $\mathscr{M}$ outputting an outcome in the set $E$ for a database $D$, and Range($\mathscr{M}$) is the co-domain of $\mathscr{M}$. 
%Differential privacy requires that the output of $\mathscr{M}$ is insensitive to the change of a single record in the input of .
%Mechanism $\mathscr{M}$ hides the presence of an individual in the data by ensuring that for any given outcome, the probability difference between  any two sibling datasets being the source of that outcome is bounded by $e^{\varepsilon}$.} 
The protection provided by DP is stronger when $\varepsilon$ approaches $0$. 
The {\em sensitivity} of a function (e.g., a query) $f$, denoted by $\Delta_f$, is the maximum amount the value of $f$ can change when adding or removing a single individual's contribution from the data. The $\varepsilon$-DP guarantee can be achieved by adding random noise derived from the Laplace distribution $\text{Lap}(\Delta_f/\varepsilon)$. For a query $f:D \rightarrow \mathbb{R}$, the {\em Laplace mechanism} (LPM) returns $f(D) + \text{Lap}(\Delta_f/\varepsilon)$, where Lap$(\Delta_f/\varepsilon)$ is a sample drawn from the probability density function Lap$(x|(\Delta_f/\varepsilon)) = (\varepsilon/2\Delta_f) \text{exp}(-|x|\varepsilon/\Delta_f)$ \cite{dwork2014algorithmic}. 

\begin{comment}
GABRIEL, CAN COMPOSABILITY PROPERTIES BE REMOVED TO SAVE SPACE ? WE DONT USE THEM ANYWHERE>
The {\em composability} property of DP helps quantify the amount of privacy attained when multiple functions are evaluated on the data. Specifically, when mechanisms $\mathscr{M}_1$, $\mathscr{M}_2$ with privacy budgets $\varepsilon_1$, $\varepsilon_2$ are applied in succession on {\em overlapping} data partitions, the {\em sequential} composition property~\cite{dwork2014algorithmic} states that the budget consumption is ($\varepsilon_1+\varepsilon_2$). Conversely, when $\mathscr{M}_1$, $\mathscr{M}_2$ are applied on {\em disjoint} data partitions, the {\em parallel} composition property states that the resulting budget consumption is $\max({\varepsilon_1, \varepsilon_2})$. The \textit{post-processing property} of differential privacy~\cite{dwork2014algorithmic} states that given any arbitrary function $h$ and an $\varepsilon$-DP mechanism $\mathscr{M}$, the mechanism $h(\mathscr{M})$ is $\varepsilon$-DP. %Lastly, we note that DP is robust to side-channel information \cite{dwork2014algorithmic}, that is, the privacy guarantee on the DP-release of $D$ is irrespective of any publicly available information about the users in $D$.}
\end{comment}

%Sensitivity is significantly influenced by whether one considers {\em event-level} or {\em user-level} privacy. In the studied case of spatio-temporal data, 
Let $f$ be a vector-valued function that outputs the population count in a location histogram at {\em every} time snapshot. With user-level privacy, removing an individual's data may cause changes in multiple elements of $f$ (in the worst case, the maximum number of reports across all individuals). Contrast this with event-level privacy, where sibling datasets differ in a single value. User-level privacy causes a significant increase in sensitivity, which must be carefully controlled to prevent utility loss.


 %At the same time, for most spatial and temporal ranges of practical interest, the number of location signals at that data point is much less than 4000XXX. 

%In this dataset, for ranges of 30 meters and 1 hour time periods, only 1 percent of the histogram cells have values more than 25. 


%\subsection{Problem Definition}\label{sec:problem_def}
\subsection{Problem Formulation}
We are given a dataset $D$ consisting of user location reports with four attributes: latitude ({\em lat}), longitude ({\em lon}), timestamp ({\em time}) and user id. The goal is to release high-resolution density information of $D$ for arbitrary spatial regions over time. We build a  $\mathbb{M}$$\times$$\mathbb{M}$$\times$$\mathbb{T}$ histogram $H$ over the data, where $\mathbb{M}$ and $\mathbb{T}$ determine the spatial and temporal resolution. $M$ and $\mathbb{T}$ are determined by application requirements, e.g., release a histogram at 30$\times$30m resolution and one hour time granularity over a duration of 24 hours~\cite{dataforgood, li2014data}. We design a mechanism $\mathscr{M}$ that takes $H$ as an input and outputs a histogram $\hat{H}$, where $\mathscr{M}$ preserves $\varepsilon$-DP.  We focus on the following three  statistical query types:

\textbf{Range count queries}. Given a query range, defined by minimum and maximum values (i.e., a range) for $lat$, $lon$ and $time$, find the number of user location reports in $D$ that satisfy this range predicate. For a query $q$, we measure the utility of its estimated DP-preserving answer, $y$, compared to the true answer $u$ using the \textit{relative error metric}, defined as $\text{RE}(y, u)=\frac{|y-u|}{\max\{u, \psi\}}$, where $\psi$ is a smoothing factor necessary to avoid division by zero.

\textbf{Nearest hot-spot queries}. Given a query location $q$ (lat, lon, time), a density threshold, $\nu$, and a spatio-temporal extent $SR$ (defined by a time duration and lengths of lat and lon geo-coordinates), find the closest cell to query $q$ within extents $SR$ that contains a number of at least $\nu$ locations signals. The hotspot query may be answered using an expanding search in the 3-d histogram until a cell within $SR$ having at least $\nu$ points is found. If none is found, the cell with the maximum count is reported. We evaluate this query in two ways: the distance penalty is measured as the Mean Absolute Error (MAE) between the true distance (as computed on $H$) and reported distance (computed on $\hat{H}$) to the hotspot. To capture hotspot density estimation errors, we measure \textit{Regret}, defined as the deviation of the reported density of the found hotspot (on noisy histogram $\hat{H}$) from the specified threshold $\nu$. Regret for a query is zero if the reported hotspot meets the density threshold. 

\textbf{Forecasting query}. Given a timeseries of density counts for a 2-d region (defined with minimum and maximum $lat$ and $lon$ values), and a forecasting horizon $h$ {\em not covered} within the timeseries, predict the count of location reports for $h$ future timesteps. To evaluate this query, we utilize \textit{holdout testing}, which removes the last $h$ data points of the timeseries, calculates the forecasting model fit for the remaining historical data, makes forecasts for $h$ timesteps, and compares the error between the forecast points and their corresponding, \textit{held-out}, data points. We report the symmetric mean absolute percentage errors (sMAPE) as $\text{sMAPE} = \frac{1}{h}\sum_{t=1}^{h}\frac{\left|F_t-A_t\right|}{(A_t+F_t)/2}$, where $A_t$ are the true counts from $H$ in the $h$ timesteps and $F_t$ are the $h$ predicted counts from a forecasting algorithm fitted to the historical data points from $\hat{H}$. 

%We evaluate the accuracy of a mechanism $\mathscr{M}$ by computing the error in answering the above queries on $\bar{H}$. We define specific error metrics for each of the queries, the details of which can be found in Sec.~\ref{sec:exp}.

%The goal is to publish $H$ while preserving differential privacy. Most methods, with a few exceptions [SNH, XX], aggregate cells in the histogram and add noise to the cells to obtain a noisy version of $H$, $\bar{H}$. Similar to [XXXX] and because of DP, we assume the queries are asked on a suitably discretized space such as a $m\times m\times t$ histogram, $H$, represented by a 3d array where each cell in the array corresponds to the number of location signals in the particular cell.


% We can assume $\bar{H}$ is also an $m\times m\times t$ histogram (or otherwise uniformity assumption can be used to obtain the desired granularity). This setup is the common implementation of DP algorithm in various system XXX, where algorithms take an $m\times m$ histogram, $H$ as input and output another $m\times m$ histogram, $\bar{H}$, which is a noisy version of $H$. 


%We study the problem of how to publish a histogram of the number of visits to each location while protecting user visit patterns. A visit pattern is defined as a sequence of locations visited by a user with timestamps. Generally, the locations visited by a user are most likely to be similar or related. Therefore, to provide a strong privacy guarantee, we propose a privacy model that can protect the user's position within a spatial-temporal window. 


\subsection{Data Characteristics and Assumptions}\label{sec:data_model}
% \label{sub:assumptions}
%SEP: I DON'T THINK THIS SHOULD BE AT THE END OF SEC. 3, BECAUSE IT RELATES BOTH TO VDR AND SYSTEM PARAMETER SELECTION. I FEEL LIKE IT SHOULD BE EITHER HERE (OR BEGINNING OF 3) OR IN 4, NOT SURE WHICH ONE IS BETTER

%\revision{In the design of VDR, we capitalize on various characteristics of real-world location datasets to be able to accurately answer spatio-temporal queries on such datasets. We first discuss two such data charctaristics that various parts of VDR design is based on.}

\revision{{\bf Density patterns.} %Our approach, VDR, relies on the existence of {\em data density patterns}. 
Real-world location datasets are generated from human mobility and tend to have similar density patterns across cities \cite{yang2015nationtelescope}, exhibiting homogeneous characteristics that capture activities like travel on road networks, visits to bars and restaurants, etc.
%A concrete example is long line segments desnity patterns in roads create, and such line segments will exist in different cities. 
%Although the actual placement of a pattern within a city may vary density values and where they are placed in a city will be different, the density in an urban location will be composed of a combination of the above patterns (IS THERE A WORD FOR IT OR A BETTER WAY OF SAYING THIS?). 
Such density patterns exist across space. For instance, areas with high density (bars, restaurant, malls) may be separated by sparse residential areas, and connected by road networks. The density patterns may also exist over time. For instance, an area that is busy on a weekend night may be less populated during a weekday afternoon (we quantify existence of temporal patterns in our datasets in Sec.~\ref{subsec:settings}). %Patterns can reoccur (1) within the same city, or (2) across cities. This is true [XXXX]. Visually, Fig.X shows roads in Houston. We see (1) repeating roads in Houston consistently create the same road patterns, and (2) we also expect that the density patterns created by road to be similar in LA or other cities. 
VDR exploits the spatial and/or temporal patterns in such datasets to achieve high accuracy %, but only requires the exisnence of spatial patterns to perform well. For instance, even in the absence of time cyclicity, VDR utilizes spatial patterns to achieve high accuracy 
compared with existing work on a broad array of real datasets, as we show in Sec.~\ref{sec:exp}. 
}
%100, 400, 1200, 4000
%80, 90, 95, 99

\noindent
\revision{\textbf{Data Distribution across users.} In real-world location datasets, the number of contributed data points varies significantly across users. While most users contribute few points, some prolific users may contribute a very large number of points. The number of points a user contributes often follows a power law \cite{muchnik2013origins, yang2015nationtelescope}. We observed this power law across all our datasets used in our experiments (see Sec.~\ref{subsec:settings}). For example, for a location dataset in Houston, the maximum number of points contributed by a user is $90,676$, while 80\%  of users have at most 100 points. This is because, in real datasets, location updates are often collected from mobile apps, with the amount of user contributions varying due to different app utilization across users. Such a power law distribution is taken into account in our statistical refinement (Sec.~\ref{sub:refinement}) to improve accuracy while accounting for user-level privacy.}





==> Spatiotemporal data release (1)/conclusion.tex <==
We proposed a technique for accurate DP-compliant release of spatio-temporal histograms that uses a combination of sampling to reduce sensitivity, VAE-based learning to counter the effect of DP-added noise, and statistical estimators to offset the effect of sampling. The resulting approach captures well spatio-temporal data patterns, and significantly outperforms existing approaches. In future work, we plan to extend our work by creating DP-compliant synthetic datasets based on spatio-temporal histograms. This is more challenging, since it needs to take into account any type of downstream processing that may be performed. One direction to achieve this goal is to sample from the compressed latent space conditioned on the time-of-day, and train a conditional image generation model such as PixelCNN~\cite{van2016conditional} over the latent pixel values.

==> Spatiotemporal data release (1)/experiments.tex <==
    % vae mae for diffeerent epsilon, basically showing learning and not overfitting.
    % transfer learning of 1 day at varying learning period.
    % transfer learning of n days from the same learning period.
    % transfer from one city to another fails: This behavior emerges because the city features the Convolution layers are used on have never been used for learning, and are therefore not present in the latent state space.
    % regularization effect of VQVAE : https://arxiv.org/pdf/1905.11062.pdf
    % im2017denoising
    % The size of codebook in the VQ-VAE controls the available options of code on rebuilding the feature maps which means that it decides how detailed the machine can reproduce the images. Thus, in the absence of noise we expect that the smaller size of codebook, the worse reconstruction results we have, and this seems the case in our test.

%We conduct an extensive evaluation of the VDR system. 
%Sec.~\ref{subsec:settings} describes the experimental testbed. Sec.~\ref{sec:exp:comparison} compares VDR with state-of-the-art approaches. Sec.~\ref{sec:exp:systemanalysis} ablates design choices. Sec.~\ref{sec:exp:ulvl} presents a case-study of a user-level density release of spatiotemporal data, and the effect of statistical refinement on answer quality. Sec.~\ref{sec:exp:patterns} showcases VDR's effectiveness for non-uniform datasets. Sec.~\ref{appx:exp} of our technical report \cite{vdr_technical} contains supplemental experimental results. 

\subsection{Experimental Settings}%\vspace{-2pt}
\label{subsec:settings}

%\subsubsection{Datasets} \label{exp:setup:dataset} We first describe all the datasets and then specify how they are utilized in our experiments.

\noindent\textbf{Datasets.} 
User check-ins are specified as tuples of: user identifier, latitude and longitude of check-in location, and timestamp. Our primary dataset is the proprietary {\em Veraset}~\cite{verasetref} data {\em(VS)}, a data-as-a-service company that collects anonymized movement data from 10\% of the cellphones in USA \cite{verasetcoverage}. For a single day in Jan 2020, there were 2.4 billion readings from 27.2 million distinct users. 

We also present results on public datasets, containing sporadic check-ins made over a relatively long period of time, as opposed to real longitudinal trajectories of users that the proprietary dataset offers. The {\em Foursquare} dataset {\em (4SQ)}~\cite{yang2019revisiting} is collected during a period of $22$ months and has 22M checkins by 114k users at 3.8 M POIs. The {\em Gowalla (GW)} dataset from the SNAP project~\cite{cho2011friendship} contains 6.4 million records from 196k unique users between February 2009 and October 2010. The {\em San Francisco taxi} dataset {\em (CABS\_SF)}~\cite{piorkowski2009crawdad} is derived from the GPS coordinates of approximately 500 taxis collected over 24 days in May 2008. 

We consider urban areas in the US covering 20km$ \times $20km each. For the Veraset data, we select cities based on their population density~\cite{pop_density}. We selected Salt Lake City, UT (VS\_SL) as a \textit{low density} city (41M points from 600k users), Los Angeles, CA (VS\_LA) as \textit{medium density} city (80M points from 852k users), and Houston, TX (VS\_HT) as high density city (221M points from 1.28M users). For all primary datasets, we discretize the temporal domain to 3 hours, giving a total of $\mathbb{T}=96$ slices for the 12 day period from Jan 7 to 19, 2020. For the secondary datasets, we discretize the temporal dimension such that each slice covers the duration of one month for a total of $\mathbb{T}=24$ slices. From the Foursquare dataset we consider its Tokyo, Japan subset (4SQ\_TKY) with 755k location updates from 8k unique users. From Gowalla we select the San Francisco (GW\_SF) subset with 568k location updates from 14k users and New York (GW\_NY) city with 520k location updates from 16k users. For the CABS dataset, following \cite{hay2016principled,qardaji2013differentially}, we keep only the start and end points of the mobility traces, for a total of 846k records. 

\noindent\revision{\textbf{Dataset Characteristics}. In all our datasets, we observed the power law distribution across users as discussed in Sec.~\ref{sec:data_model}. Summary power law statistics and visualizations are presented in Sec.~\ref{appx:data_charactaristics}. To quantify the existence of temporal patterns, we extracted density timeseries for each of the $\mathbb{M}\times\mathbb{M}$ cells in the histogram % count data over 8-12 days at all ($\mathbb{M}\times\mathbb{M}$) cells, 
and evaluated an Autocorrelation Function (ACF) on the  timeseries. We found that only 6.2\% (VS\_HT), 2.4\% (VS\_LA), and 1.5\% (VS\_LA) of such series exhibit non-stationarity, showing that for most cells, we do not observe such temporal patterns. }

% no space for table % Table \ref{tbl:cities} summarizes the datasets.
\noindent\textbf{Parameter Settings.}
Following \cite{dataforgood,li2014data, zhang2016privtree}, we partition the space into a $576$$\times$$576$ (i.e., $\mathbb{M}=576$) grid to obtain $30m\times30m$ cells. As described above, the temporal granularity is specific to each dataset. The default value of privacy budget $\varepsilon$ is set to $0.2$.

\noindent\textbf{Evaluation Metrics.} For range count queries, we construct query sets of 5,000 RCQs centered at randomly selected data records. Each query has side length that varies uniformly from 30 meters to 120 meters. We set smoothing factor $\psi$ to 0.1\% of the cardinality $n/\mathbb{T}$ of the average time slice of the spatio-temporal dataset~\cite{zhang2016privtree,cormode2012differentially,qardaji2013differentially}. When comparing multiple datasets with each other, the smallest smoothing constant among them is used to remain consistent. 

We evaluate forecasting queries on Veraset subsets only, since other datasets do not contain timeseries of sufficient length. \revision{In order to find forecastable timeseries in the majority of queries, we sampled positions of POIs in the city and extracted timeseries of random lengths that satisfy a ACF Seasonality test~\cite{makridakis2000m3} (90\% confidence) at seasonal period of 8 (meaning a daily seasonality according to 3 hour temporal discretization of the 24 hour period)}.
%if you relax the test then Houston, Los Angeles, Salt Lake 10\%, 4\%, 2\%, respectively.
% For instance, in VS\_HT 90\% of such series daily seasonality (repeating every 8 timesteps according to 3 hour temporal discretization of the 24 hour day) as tested by an Autocorrelation Seasonality test\cite{makridakis2000m3} (90\% confidence). 
To make forecasts, we use the winning algorithm of the M3 forecasting competition~\cite{makridakis2000m3}, Theta~\cite{assimakopoulos2000theta}, which is a variant of the Simple Exponential Smoother.
%with additional heuristics to fit seasonality and trends within a timeseries. For each timeseries for the forecasting query, we use Maximum Likelihood Estimation to the fit the forecasting model over 
We use the data of all-but-last day to fit the forecaster and evaluate its predictions for last day (i.e., a horizon of $h=8$). We report the sMAPE error (Sec.~\ref{sec:bck}) on 100 forecastable timeseries.
% We report the symmetric mean absolute percentage errors (sMAPE) as $\text{sMAPE} = \frac{1}{h}\sum_{t=1}^{h}\frac{\left|F_t-A_t\right|}{(A_t+F_t)/2}$, where $A_t$ are the true counts and $F_t$ are the forecasted counts.

Lastly, the hotspot query is evaluated at a specified threshold $\nu$. Queries originating at random from 1000 randomly selected data points are answered using an expanding search within the 3-d spatial region $SR$ with lengths 5km in spatial extent and no bounds in the time dimension.

\noindent\textbf{Implementation.}  All algorithms were implemented in Python, and executed on Linux machines with Intel i9-9980XE CPU, 128GB RAM and a RTX3090 GPU. Neural networks are implemented in JAX~\cite{jax2018github}. Given this setup, VDR took up to 50 minutes to train for 12 days of the Veraset Houston data. The inference time of VDR is less than 1ms and the model takes 9 MB of space. We publicly release the source code at~\cite{vdr_implementation}.


\noindent\textbf{Model Training.} For Multi-Resolution Learning we augment the training set at $r=3$ granularities chosen at equal spacing between the minimum (30m) and maximum (120m) query ranges to be evaluated. The encoder and decoder architecture is based on ResNet\cite{targ2016resnet}. The model takes as input batches of histogram slices and passes them through the ConvNet encoder $\theta_e$ and decoder $\theta_d$. 
\revision{The choice of VAE is primarily motivated by faster training times and often better accuracy for datasets with multiple slices. In Figure~\ref{fig:gpvae_vs_vqvae} we compare a Gaussian-Process VAE (which learns a continuous latent variable) to the Vector-Quantized VAE as used in VDR (which learns a discrete latent variable, i.e., a codebook). For the models to achieve their lowest error, we observe that VQ-VAE requires a lower number of epochs on both public (CABS\_SF) and proprietary (VS\_HT) datasets. The gap is notable in VS datasets due to them having a larger number of slices to train on, which are in-addition multiplied by Multi-Resolution Learning. In such instances, VQ-VAE is able to both train quicker and achieve better accuracy. To train the VQ-VAE, we utilize the Adam~\cite{kingma2014adam} optimizer with Exponential Moving Average updates \cite{razavi2019generating}. The EMA version trained much faster than the non-EMA version, especially when using MRL. Using EMA updates also has the advantage that the embedding updates are independent of the choice of optimizer used for the encoder, decoder and other parts of the architecture.} 
\revision{The loss function used to train the codebook is as in \cite{van2017neural}}.
 In all our experiments, we utilize hyperparameters consistent with those utilized in previous work~\cite{van2017neural,razavi2019generating}; i.e., $\ell=64$, $\mathcal{B}=128$ and a batch size of $b=8$. \revision{ $\alpha$ is used only to study the impact of regularization on model robustness and is set to 1 (equal weighting).}


\begin{figure}
    %\centering
    \begin{minipage}[t]{0.45\linewidth}
        \includegraphics[width=\linewidth]{other_figures/epochs_vs_accuracy_cabs}
    \end{minipage}
    \begin{minipage}[t]{0.45\linewidth}
        \includegraphics[width=\linewidth]{other_figures/epochs_vs_accuracy_vsht}
    \end{minipage}   
    \caption{Choice of Variational AutoEncoder}
    \label{fig:gpvae_vs_vqvae}
    \vspace{-5pt}
\end{figure}

\vspace{-2pt}

\subsection{Comparison with Baselines} \label{sec:exp:comparison}
\noindent\textbf{Baselines.}
We use as benchmarks  Uniform Grid (UG) \cite{qardaji2013differentially}, Adaptive Grid (AG) \cite{qardaji2013differentially}, HB\_striped \cite{zhang2018ektelo,qardaji2013understanding}, PrivBayes~\cite{zhang2017privbayes}, AHP~\cite{zhang2014towards} and MWEM~\cite{hardt2012simple}. Brief summaries of each method are provided in Sec.~\ref{sec:rel_works}. We utilize Ektelo \cite{zhang2018ektelo,ektelogit}, an operator-based framework for implementing privacy algorithms. To extend approaches designed to originally support range queries in two-dimensional data (spatial-only) to the 3-d case, we partition the temporal domain into non-overlapping slices, so that the measurements are essentially the 2D histograms resulting from each slice. For example, HB\_striped\cite{zhang2018ektelo} performs on each slice the HB algorithm \cite{qardaji2013understanding}, which builds an optimized hierarchical set of queries. We similarly implement Uniform Grid (UG)\cite{qardaji2013differentially} and Adaptive Grid (AG)\cite{qardaji2013differentially}. We use as-is algorithms that are designed to extend to the multi-dimensional setting such as PrivBayes~\cite{zhang2017privbayes}, AHP~\cite{zhang2014towards} and MWEM~\cite{hardt2012simple}. 
%Lastly, we also considered QuadTree \cite{cormode2012differentially}, but the results were far worse than the above approaches and thus are not reported. 
We were unable to run the DAWA \cite{li2014data} algorithm directly on such a large domain due to memory and computational constraints. DAWA is designed for 1D-inputs and extended to 2D using a Hilbert fractal. 

\textbf{Privacy Model}. Since none of the baselines consider user-level privacy, to allow for a fair comparison we present experiments with event-level privacy. We disable VDR's sampling and statistical refinement steps, and assume each record belongs to a separate user, hence the privacy protection offered degrades to event-level. We evaluate VDR with user-level privacy in Sec.~\ref{sec:exp:ulvl}.

\vspace{-8pt}
\subsubsection{Range Count Query}

\begin{figure*}
    %\centering
    \begin{minipage}[t]{\textwidth}
        \includegraphics[width=\textwidth]{other_figures/rcq4cities_re20.eps}
        \vspace{-5mm}
        \caption{Impact of privacy budget on range count query (RCQ) accuracy.}
        \label{fig:rcq}
    \end{minipage}  
    \vspace{-5mm}
\end{figure*}

\begin{figure*}
    %\centering
    \begin{minipage}[t]{0.375\textwidth}
        \includegraphics[width=\textwidth]{fcast_figures/rcq_varyrange_re20.eps}
        \vspace{-3mm}
        \caption{Impact of query size on RCQ.}
        \label{fig:qsize}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.615\textwidth}
        \includegraphics[width=\textwidth]{fcast_figures/fcast_SMAPE.eps}
        \vspace{-3mm}
        \caption{Impact of privacy budget on  forecast query error (sMAPE)}
        \label{fig:fcast}
    \end{minipage}  
    \vspace{-5mm}
\end{figure*}

\begin{figure*}
    %\centering
    \begin{minipage}[t]{\textwidth}
        \includegraphics[width=\textwidth]{fcast_figures/hotspot_nyhtla_hot20_revised}
    \vspace{-5mm}
    \caption{Impact of privacy budget on hotspot query accuracy.}
    \label{fig:hotspot_threshold20}
    \end{minipage}  
    \vspace{-2mm}
\end{figure*}

Figure ~\ref{fig:rcq} presents the error of VDR and the compared approaches when varying $\varepsilon$ (smaller $\varepsilon$ means stronger privacy protection). Unsurprisingly, the error reduces as $\varepsilon$ increases, with VDR consistently outperforming all competitor approaches. VDR is effective in capturing spatial patterns from the data and using them to smooth excessive noise. 

Figure~\ref{fig:qsize} evaluates the impact of query size on accuracy for datasets GW\_NY and VS\_HT (similar trends were observed for other datasets). The error increases when query size grows, due to the fact that computing the result requires aggregating more grid cells, each contributing additional error to the answer. Still, VDR consistently outperforms competitors at all query sizes. 


\subsubsection{Forecasting Query}
Figs.~\ref{fig:fcast}(a)-(c) show results on Veraset data subsets VS\_HT, VS\_LA and VS\_SL (corresponding to high, medium and low density). Remarkably, for $\varepsilon=0.2$ and higher, VDR performs as well as the non-private benchmark (`No Noise'). VDR is robust to density changes in the data, as its performance is not significantly different across the three datasets.
VDR significantly outperforms all private benchmarks, with its ability to smooth out the noise. In some instances, e.g., $\varepsilon=0.05$ of Fig~\ref{fig:fcast}(c), UG can perform well, but it does so by making \textit{naive} forecasts that predict the last period's actuals as next period's value, without establishing causal factors.


\vspace{-3pt}

\subsubsection{Hotspot Query}
Fig.\ref{fig:hotspot_threshold20} reports the accuracy for hotspot queries on various Veraset subsets at the fixed density threshold of $\nu=20$. We report the results for varying thresholds in Sec.~\ref{appx:exp} of our technical report~\cite{vdr_technical}.
Mechanisms that model directly the data distribution such as MWEM, AHP and PrivBayes tend to underestimate density globally, and incur a large MAE and regret penalty, up to the maximum of the density threshold. To the same effect, UG, due to its coarse partitioning of the data domain, underestimates the `hot' peaks that the query searches for, also experiencing both a large MAE and regret. AG improves these estimates to some extent by building a finer domain partitioning in the lower level of its hierarchy, and while it may not locate the closest hotspot (high MAE), it still finds one that meets the density threshold (lower regret). LPM fares well for this query as it is not affected by the biases that partitioning approaches bring about. VDR further improves on LPM in both metrics.  In all instances, VDR finds an effective balance between the MAE and regret error metrics.

By starting with an unbiased estimate of the density counts and denoising them, VDR clearly outperforms the existing state-of-the-art in all settings. Next, we no longer consider competitor approaches, and we focus on analyzing the behavior of VDR when varying system parameters. 


\subsection{System Analysis}\label{sec:exp:systemanalysis}
\begin{figure*}
    \centering
        \begin{minipage}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{other_figures/regularization_vs_modelsize.eps}
        % \vspace{-2mm}
        \caption{Model regularization analysis}
        \vspace{-2mm}
        \label{fig:regularization_analysis}
    \end{minipage} 
    \hfill
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{other_figures/learningslices_vs_modelsize.eps}
        % \vspace{-2mm}
        \caption{Learning Period Analysis}
        \vspace{-2mm}
        \label{fig:learningperiod_analysis}
    \end{minipage}
        \hfill
    \begin{minipage}[t]{0.24\textwidth}
\includegraphics[width=\textwidth]{other_figures/data_augmentation_analysis.eps}
        % \vspace{-2mm}
        \caption{Benefits of Multi Resolution Learning}
        \vspace{-2mm}
        \label{fig:mrl_comparison}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\textwidth}
\includegraphics[width=\linewidth]{other_figures/varying_temporal_resolution_all_cities}
        \caption{Effect of varying temporal resolution}
        \vspace{-2mm}
    \label{fig:temporal_resolution}
    \end{minipage}
\end{figure*}

\begin{figure}
    \begin{minipage}[t]{0.46\linewidth}
            \includegraphics[width=\textwidth]{other_figures/transfer_accuracy_vs_learning_period.eps}
        % \vspace{-7mm}
        \caption{Impact of varying learning period}
        \label{fig:transfer_learning1}
        
    \end{minipage} 
    \hfill
    \begin{minipage}[t]{0.46\linewidth}
            \includegraphics[width=\textwidth]{other_figures/transfer_accuracy_over_period.eps}
        % \vspace{-7mm}
        \caption{Out-of-sample denoising.}
        \label{fig:transfer_learning2}        
    \end{minipage}
    % \vspace{-10pt}
\end{figure}

\subsubsection{Modeling choices\nopunct}\label{subsec:system_modelling}\hfill\\
\noindent\textbf{Effect of model regularization on performance}.
We evaluate the effectiveness of \textit{Variational-AutoEncoders} in denoising DP histograms. Recall that,  by training a lower dimension representation of the data, we wish to learn patterns without overfitting to the noise. In Fig.~\ref{fig:regularization_analysis} we evaluate VDR against `R. focus', a method that simulates an AutoEncoder by over-emphasizing reconstruction loss (i.e., by setting $\alpha$ to a very small value). We consider both public and proprietary datasets while varying the bottleneck size. We notice that a small bottleneck performs poorly due to having limited representation power to learn the input data. When increasing the bottleneck, we see polar effects in the presence and absence of regularization. In the case of `R. Focus', the model quickly overfits to the noise, decreasing accuracy. Whereas if the AutoEncoder is sufficiently regularized, accuracy remains good even for large models due to the learning of generalizable patterns, emphasizing the need for regularizing the encoding space. 

% made clear that bottleneck size and regularization loss and separate but complementing types of regularization effects.

\noindent\textbf{Effect of learning period}.
%We study how learning period affects the accuracy of our method. F
Fig.~\ref{fig:learningperiod_analysis} shows the accuracy of denoising when 
we train the VAE with a varying number of slices. When the number of learning slices is one, we have in essence a snapshot dataset in 2D. As we add more slices to training, the learning is stabilized and the the learned patterns help achieve better denoising performance in the entire dataset.
% relate the number of learning slices to the bottleneck size in a more formal wya



\noindent\textbf{Effect of Multi Resolution Learning on accuracy}.
%Fig.~\ref{fig:mrl_comparison}, we ablate Multi-Resolution Learning (MRL). 
Fig.~\ref{fig:mrl_comparison} shows that across all datasets, by augmenting the training set with coarser granularity histograms, we learn a model that can answer queries more accurately. This is also due to the smoothing effect of the ConvNet, as learned information from one slice helps denoise another within the same dataset.

\noindent\textbf{Effect of Temporal Resolution}.
\revision{We evaluate the accuracy of VDR at several granularities of discretization of the temporal domain. For the 12 day period that each Veraset dataset covers, varying the time duration also varies the number of slices each dataset produces; from as many as 576 (for 22 minutes per slice) to 12 (for 24 hours per slice). Figure \ref{fig:temporal_resolution} shows the accuracy of VDR on all Veraset datasets at privacy budgets of 0.1 and 0.4. Accuracy improves as the temporal resolution becomes coarser. Given that the number of points in the dataset is fixed, there are two compounding effects of increasing the temporal duration per slice. The first increases the number of points in each slice, causing the \textit{relative} error to plummet because the denominator (true answer) grows in value. In addition, the denoising ability of VDR improves with coarser temporal resolution since (1) each slice contains more defined spatial patterns due to longer time aggregation and (2) slices tend to become similar to each other, and the repeating patterns are now easier to summarize for the bottleneck layers of the VAE.}
%A more interesting comparison is when looking at the mean absolute error in Figure \ref{fig:temporal_resolution}(b). Since the magnitude of noise in a LPM mechanism is constant, all LPM lines hover around MAE of 5, corresponding to average noise of random variable sampled from Laplace distribution scaled to $1/\varepsilon$.

% \begin{figure}
%     \begin{minipage}[t]{0.48\linewidth}
%         \includegraphics[width=\linewidth]{other_figures/varying_temporal_resolution_re}
%         % \caption{Relative Error}
%         % \label{fig:tr_re}
%     \end{minipage}
%         \hfill
%     \begin{minipage}[t]{0.48\linewidth}
%         \includegraphics[width=\linewidth]{other_figures/varying_temporal_resolution_mae}
%         % \caption{MAE Error}
%         % \label{fig:tr_mae}
%     \end{minipage}
%     \caption{Effect of varying temporal resolution}
%     \label{fig:temporal_resolution}
%     % \begin{minipage}[t]{0.18\textwidth}
%     % \end{minipage}
%     % \label{fig:gmm}
% \end{figure}




% \vspace{-3pt}
\subsubsection{Data release over time}
We study the effectiveness of VDR when releasing data over time. Specifically, we measure how often VDR needs to be retrained when new data arrive. For this experiment we utilize the Veraset Houston data for a period of 24 days, with each slice representing a one hour time period.  We consider a training period, $T_b$ to $T_e$, where $T_b$ is the beginning of the training period and $T_e$ is the end, and a testing period that starts at $T_e$ and ends at $T_t$. We refer to the period $T_b$ to $T_e$ as in-sample and $T_e$ to $T_t$ as out-of-sample. We evaluate the performance of the model in two scenarios. In Figure \ref{fig:transfer_learning1}, we test the denoising performance of VDR on an out-of-sample period of 3.5 days (84 slices). VDR in-sample and out-of-sample show the accuracy of VDR on the in-sample and out-of-sample period, respectively. The training data period is varied by moving $T_b$ forward in time but keeping $T_e$ and $T_t$ the same (so training period ranges from 420 to 12 slices). Performance first improves when the training period is up to 3.5 days, as having more data helps the model denoise via better generalizabilty. But as even more data is used in the training, specificity of the patterns is reduced, hence accuracy suffers. In the second setting (Fig.~\ref{fig:transfer_learning2}), we train VDR over slices of `TP' (\textit{Training period}) number of days, and use the trained model to denoise. For in-sample testing the {\em Transfer Period} refers to the accuracy of VDR on the training data itself. We see that the model accuracy is mostly unaffected. For out-of-sample testing \textit{Transfer} period refers to the number of days from $T_e$ to $T_t$. We increase $T_t$ so that transfer period ranges from 1 day to 9 days. We see that performance degrades when denoising out-of-sample periods far from the training periods. We recommend retraining of the VAE model every couple of days.

%\vspace{-3pt}

\subsection{User-level privacy and statistical refinement}\label{sec:exp:ulvl}

\begin{figure}
    \centering
    \begin{minipage}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{other_figures/ulvl_NE_SE_vs_SR.eps}
        \vspace{-2mm}
        \caption{Sampling and Noise Error trends.}
        \label{fig:NEvsSE}
    \end{minipage} 
    \hfill
    \begin{minipage}[t]{0.23\textwidth}
        \includegraphics[width=1\textwidth]{other_figures/ulvl_NN_id_vs_g.eps}
        \vspace{-2mm}
        \caption{Effect of Scaling factor $g$ on SE and SE+NE }
        \label{fig:debiasing_factor}
    \end{minipage}
    \vspace{-2pt}
\end{figure}
\begin{figure}
    \centering
    \begin{minipage}[t]{0.22\textwidth}
    \includegraphics[width=\textwidth]{other_figures/ulvl_vdr_vs_C.eps}
    \vspace{-2mm}
    \caption{Varying refinement constant $C$ for VDR.}
    \label{fig:vdr_vs_debiasingC}
    \end{minipage}
    \hfill
     \begin{minipage}[t]{0.22\textwidth}
        \includegraphics[width=\linewidth]{other_figures/ulvl_growth_ratio}
        \vspace{-2mm}
        \caption{Varying growth ration $\lambda$ for VDR}
        \label{fig:ulvl_growthratio}
    \end{minipage}
    \vspace{-2pt}
\end{figure}

We consider several Veraset data subsets, and set $\varepsilon=6$, analogous to~\cite{aktay2020google, chang2021mobility}. Recall that, in order to release data without consuming excessive privacy budget, we bound the maximum number of contributions of a user to $k$, consequently having access to only the sampled subset $D_s$ to learn our model. Note that in Figs.~\ref{fig:NEvsSE}, \ref{fig:debiasing_factor}, \ref{fig:vdr_vs_debiasingC} and \ref{fig:vdr_debias_performance} the relative error metric is evaluated w.r.t to the true data $D$, while the query computations are performed over $D_s$. 


\subsubsection{Challenges for User-Level Privacy}\label{subsec:ulvlchallenges} \revision{We first empirically validate the discussion in Sec.~\ref{sub:collection} and Sec.~\ref{sub:refinement} regarding challenges for user-level privacy without using VDR.}

\noindent\textbf{Bounding user contribution.} \revision{In Fig~ \ref{fig:NEvsSE} we focus on bounding user contributions to achieve good accuracy.} The experiment evaluates the accuracy of answering range count queries  when varying the sampling rate $k$. Sampling error (denoted as SE) measures the error induced purely due to bounding the contribution of each user to $k$. As expected, SE decreases as the sampled subset $D_s$ comes closer to representing the true dataset $D$.
%(also refer to Fig.~\ref{fig:stats}). We also report the error in the DP-preserving answer using LPM. Denoted by $SE+NE$ is LPM which contains errors induced due to DP-compliant noise in addition to those due to sampling. As $k$ increases, the benefits from increased sampling dominate the total effect (see $k = 2 \text{ to } 16$), however the sensitivity of the query (hence, the noise) eventually exceeds the rate at which sampling error decreases, causing a sharp increase in the error of the reported answer (see $k = 32$ to $256$). 
%The minimum of the total error is reached at different values of $k$ depending on the characteristics of user participation in that dataset. Thus, there is an ideal value of $k$, and 
%We discuss how to set the ideal value of $k$ at the end of this section.

\noindent\textbf{Analysing the effects of brute-force debiasing.} \revision{In Fig~ \ref{fig:debiasing_factor} we show that without VDR, debiasing by scaling the query answers leads to poor accuracy, as discussed in Sec.~\ref{sec:refine:challanges}.} Recall that the answer to the range count query reported on $D_s$ can be scaled according to $N/n$ to potentially debias the result. However, since the data is skewed and with added noise, such a scaling affects the results negatively. We vary the degree of scaling as $g\times N/n$ for values of $g$ from 0.1 to 1. Figure \ref{fig:debiasing_factor} shows that for sampling induced error SE, scaling the answer can be useful. However, after adding DP-compliant noise (plot line SE+NE), upscaling also amplifies the noise in the reported counts and almost always yields poor accuracy. Therefore, to utilize any form of scaling it is important to first denoise the data, as done in VDR.


\subsubsection{VDR System Parameters}\label{sec:exp:ulevel:params}
\revision{Before being able to use VDR to address the above challenges, we need to set the two system parameters: refinement factor $C$ and growth ratio $\lambda$. We empirically validate our guidelines for setting the two parameters here.}

\textbf{Refinement Factor, $C$}. \revision{ In VDR, the denoised histogram is scaled according to the proposed statistical refinement step, in order to offset the effects of sampling at $k$ points per user. The refinement constant $C$ determines, according to Eq.~\eqref{eq:gamma}, the degree of scaling $\gamma$ that is applied to the query answer. For example, at $C=1$, $\gamma$ approaches $N/n$, equivalent to a basic scaling of the query answer. } In Figure \ref{fig:vdr_vs_debiasingC}, we evaluate the accuracy of VDR while varying $C$ at various degrees of sampling $k$. Remarkably, among all settings the lowest error is achieved at $C=5\text{e-5}$, substantiating our claim that a fixed value of $C$ is sufficient to refine answers. \revision{The suitability of a fixed value constant is owing to the fact that human mobility has similar characteristics across cities, as discussed in Sec.~\ref{sec:data_model}. Thus, we recommend to set $C=5\text{e-5}$ across all datasets.}


\textbf{Growth Ratio, $\lambda$}. \revision{Recall that VDR samples $k$ points per user, where $k=\lambda N$ and $\lambda$, the growth ratio, is a system parameter.  In Fig.~\ref{fig:ulvl_growthratio} we vary the growth ratio for several datasets including datasets assumed public for the sake of privacy accounting, VS\_MW (Milwaukee) and VS\_MI (Miami). The results show that across all datasets, similar growth ratio achieves the best accurcy. This confirms that, due to similarity in skewness inherent to location datasets (discussed in Sec.~\ref{sec:data_model}), the same value of $\lambda$ performs well across datasets. Thus, we recommend setting $\lambda = 2.5\text{e-7}$. }




\begin{figure}
\centering
    %\begin{minipage}[t]{0.5\textwidth}
        %\includegraphics[width=0.5\linewidth]{other_figures/ulvl_growth_ratio}
        %\caption{Learning behavior with growth ratio %of sampled dataset}
        %\label{fig:ulvl_growthratio}
        \includegraphics[width=0.7\linewidth]{other_figures/ulvl_VDRatC_vs_SR.eps}
        %\vspace{-3mm}
        \caption{Benefit of VDR refinement }
        \label{fig:vdr_debias_performance}
        %\end{minipage}
          \vspace{-2pt}
\end{figure}


\begin{figure*}
\centering
    \begin{minipage}[t]{0.48\textwidth}
\centering
        \includegraphics[height=2.3cm]{gmm/conv_vae_recon_7_gmm0.35.png}
        % \vspace{-10pt}
        \caption{Learning behavior at GMM $\sigma=3$}
        \label{fig:gmm3}
    \end{minipage}
        \hfill\begin{minipage}[t]{0.48\textwidth}
\centering
        \includegraphics[height=2.3cm]{gmm/conv_vae_recon_7_gmm0.65.png}
        % \vspace{-10pt}
        \caption{Learning behavior at $\sigma=7$}
        \label{fig:gmm7}
    \end{minipage}
    \begin{minipage}[t]{0.18\textwidth}
    \end{minipage}
    \label{fig:gmm}
    \vspace{-5pt}
\end{figure*}


\begin{figure}
\begin{minipage}[t]{0.2\textwidth}
        \includegraphics[width=\textwidth]{other_figures/gmm_varying_sigma.eps}
        % \vspace{-8mm}
        \caption{Varying $\sigma$}
        \label{fig:gmm_variance}
        \end{minipage} 
        \hfill
    \begin{minipage}[t]{0.20\textwidth}
        \includegraphics[width=\textwidth]{other_figures/gmm_varying_bottleneck.eps}
        % \vspace{-8mm}
        \caption{Varying $\mathcal{B}$.}
        \label{fig:gmm_bottleneck}
    \end{minipage}
    \vspace{-2pt}
\end{figure}


\subsubsection{VDR Refinement}  In Fig.~\ref{fig:vdr_debias_performance} we compare VDR with the approach that reports the answer computed on $D_s$ as-is. In all datasets, there is a clear benefit to using statistical refinement, improving the error by up to 40\% in the case of VS\_HT, a high density city. 
%VDR with its denoising ability welcomes itself to the refinement of implicit sampling errors. 

 \revision{We conclude with evaluating our heuristic on setting $k$ as  $k=\lambda N$, discussed in Sec.~\ref{sec:system:trade-offs}.  The heuristic, based on the growth ratio $\lambda=2.5\text{e-7}$, empirically determined in Sec.~\ref{sec:exp:ulevel:params},} recommends setting $k= 10$ for VS\_SL, $k=20$ for VS\_LA and $k=53$ for VS\_HT. As we see in Fig.~\ref{fig:vdr_debias_performance}, these values of $k$ achieve close to the best accuracy for their corresponding cities, validating our heuristic for setting $k$ as a constant fraction of data size.


% From Fig.~\ref{fig:vdr_debias_performance} we see that the best accuracy in VS\_LA is achieved at $k=16$ ( for the growth ratio . For the same value of $\lambda$, we get for VS\_SL,  
% $k*=8.81$ ($N=44\text{M}$) and for VS\_HT, $k*=44$ ($N=221\text{M}$). T


% \vspace {-3pt}

\subsection{Learning Ability on Non-Uniform Datasets}\label{sec:exp:patterns} 


%We study the ability of VDR to learn spatial patterns from noisy observations in skewed datasets.

\noindent\textbf{Setup}. We synthesize $2M$ points from a Gaussian Mixture Model (GMM) \cite{reynolds2009gaussian} with 50 components positioned at random in the 3D integer lattice $\mathbb{Z}^3$ of size $9$$\times$$9$$\times$$9$. All components are equally weighted and have the covariance matrix $\vec{I}\times\sigma^2$, where $\vec{I}$ is the identity matrix. To control the variation around its mean value, we adjust the parameter $\sigma$. \revision{For clarity of visualization, we partition the synthetic data} into a 3D histogram of 100$\times$100$\times$100 cells. We train and denoise with VDR on the 100 slices. 
We report $\sigma$ in terms of the number of such cells, with a smaller variance implying a data spread tighter around the mean of each GMM component, thus mimicking the skewed data distributions typically present in spatio-temporal location datasets. Fig.~\ref{fig:gmm3} ($\sigma=3$) and Fig.~\ref{fig:gmm7} ($\sigma=7$) visualize a single slice of this dataset with its true values (left), noisy data collections (middle) and denoised reconstructions (right). VDR has a strong ability to recover the underlying patterns of GMMs from even highly distorted observations.
\revision{Moreover, Figure \ref{fig:gmm_variance} ($\varepsilon = 0.2$) shows that as we increase the variance $\sigma^2$ of the GMM components, the model performance suffers, since at a large variance (e.g., Fig.~\ref{fig:gmm7}) data is more uniformly distributed and lacks the spatial patterns typically exhibited in location datasets (such as those depicted in Figure \ref{fig:histogram_overtime}). }
% We report $\sigma$ in terms of the number of such cells, with a smaller variance implying a data spread tighter around the mean of each GMM component, thus mimicking the skewed data distributions typically present in spatio-temporal location datasets. Fig.~\ref{fig:gmm3} ($\sigma=3$)
% %and Fig.~\ref{fig:gmm7} ($\sigma=7$)  
% visualizes a single slice of this dataset with its true values (left), noisy data collections (middle) and denoised reconstructions (right). VDR has a strong ability to recover the underlying patterns of GMMs from even highly distorted observations.
% Moreover, \revision{In Figure \ref{fig:gmm_variance} ($\varepsilon = 0.2$) we simulate two extremes of data spread. On one extreme, we simulate the absence of any spread by concentrating all points belonging to a GMM at its center (in a single cell for $\sigma=0.01$). The denoising ability of VDR is compromised because in the absence of spatial spread patterns---such as those depicted in Figure \ref{fig:histogram_overtime}---to exploit, VDR resolves to simply learning the counts reported directly from LPM, and the only advantage stems from denoising in empty regions. On the other extreme, we simulate data that is more uniformly distributed and also lacks distinct the spatial patterns typically exhibited in location datasets (increasing $\sigma$ to 6). At a large variance,
% %(such as the one depicted in Fig.~\ref{fig:gmm7})
% the model performance suffers overall, since distinct repeatable patterns are not present even though VDR can denoise effectively.}
Lastly, we evaluate the effect of varying the bottleneck size of the VAE on the learning ability of VDR. Figure \ref{fig:gmm_bottleneck} shows that, for a given privacy budget, a larger bottleneck is required to capture more skewed datasets. When data are skewed (compare lines for $\varepsilon=0.1$ and $\varepsilon=0.8$ at $\sigma=1$), less DP noise in the data collection step helps further emphasize the data spread, benefiting from having a larger model capacity to learn precisely such patterns. 
%We conclude by stating that VDR is especially capable of learning spatial-like patterns in the data where present, utilizing them to denoise effectively. 

% instead of saying tha tulevel setting requires a grid search
% it has to be calibrated as a fucntion of sampling rate to the total dataset size N. If larger data then 



% \begin{figure*}[t]
%     \centering
%     \vspace{-10mm}
%     \subfloat{
%     \includegraphics[height=2.5cm]{gmm/conv_vae_recon_7_gmm0.35.png}}

%     \subfloat{
%     \includegraphics[height=2.5cm]{gmm/conv_vae_recon_7_gmm0.55.png}    }
    
%     \subfloat{
%     \includegraphics[height=2.5cm]{gmm/conv_vae_recon_7_gmm0.65.png}    }
    
%     \subfloat{
%     \includegraphics[height=2.5cm]{gmm/conv_vae_recon_7_gmm0.95.png}    }
%     \caption{Gaussian Mixture Model visualization at $\sigma$ varying from 3(top), 5, 7, 9(bottom)}
%         \label{fig: timeline}
% \end{figure*}


% \begin{figure}
%  \centering
%  \begin{subfigure}[b]{0.7\textwidth}
%      \centering
%      \includegraphics[width=\textwidth]{gmm/conv_vae_recon_7_gmm0.35}
%      \caption{$\sigma=0.35$}
%  \end{subfigure}
%  \vspace{-2mm}
%  \hfill
%  \begin{subfigure}[b]{0.7\textwidth}
%      \centering
%      \includegraphics[width=\textwidth]{gmm/conv_vae_recon_7_gmm0.55}
%      \caption{$\sigma=0.55$}
%  \end{subfigure}
%  \vspace{-2mm}
%  \hfill
%  \begin{subfigure}[b]{0.7\textwidth}
%      \centering
%      \includegraphics[width=\textwidth]{gmm/conv_vae_recon_7_gmm0.65}
%      \caption{$\sigma=0.65$}
%  \end{subfigure}
%  \vspace{-2mm}
%  \begin{subfigure}[b]{0.7\textwidth}
%      \centering
%      \includegraphics[width=\textwidth]{gmm/conv_vae_recon_7_gmm0.95}
%      \caption{$\sigma=0.95$}
%  \end{subfigure}
% \caption{}
% \label{fig:gmm_vis}
% \vspace{-2mm}
% \end{figure}




% RCQ figyures ehrere
% \begin{figure*}
%     %\centering
%     \begin{minipage}[t]{0.25\textwidth}
%         \includegraphics[width=\textwidth]{rcq_figures/4SQ_TOKYO_re40}
%         \vspace{-2mm}
%     \end{minipage}    
%     \hspace{-2mm}
%     \begin{minipage}[t]{0.25\textwidth}
%         \includegraphics[width=1\textwidth]{rcq_figures/CABS_SF_re40}
%         \vspace{-2mm}
%     \end{minipage}   
%     \hspace{-2mm}
%     \begin{minipage}[t]{0.25\textwidth}
%     \includegraphics[width=\textwidth]{rcq_figures/GW_SF_re40}
%     \vspace{-2mm}
%     \end{minipage}
%     \hspace{-2mm}
%     \begin{minipage}[t]{0.25\textwidth}
%     \includegraphics[width=\textwidth]{rcq_figures/GW_NY_re40}
%     \vspace{-2mm}
%     \end{minipage}
%     \hspace{-2mm}
%     \label{fig:rcq_auxdata}
%     \caption{Range Count Query answer at varying spatial ranges.}
% \end{figure*}


% \begin{figure*}
%     %\centering
%     \begin{minipage}[t]{0.29\textwidth}
%         \includegraphics[width=\textwidth]{rcq_figures/VS_HOUSTON_re40}
%         \vspace{-2mm}
%     \end{minipage}    
%     \begin{minipage}[t]{0.29\textwidth}
%         \includegraphics[width=1\textwidth]{rcq_figures/VS_LOSANGELES_re40}
%         \vspace{-2mm}
%     \end{minipage}        
%     \begin{minipage}[t]{0.29\textwidth}
%     \includegraphics[width=\textwidth]{rcq_figures/VS_SALT_LAKE_re40}
%     \vspace{-2mm}
%     \end{minipage}
%     \label{fig:rcq_vsdata}
%     \caption{Range Count Query answer at varying spatial ranges.}
% \end{figure*}



% \begin{figure*}
%     %\centering
%     \begin{minipage}[t]{0.18\textwidth}
%         \includegraphics[width=\textwidth]{rcq_figures/QSIZE_4SQ_TOKYO_re40}
%         \vspace{-2mm}
%         \label{fig:modeling}
%     \end{minipage} 
%     \hspace{-2mm}
%     \begin{minipage}[t]{0.18\textwidth}
%         \includegraphics[width=1\textwidth]{rcq_figures/QSIZE_CABS_SF_re40}
%         \vspace{-2mm}
%         \label{fig:uniformity}
%     \end{minipage}  
%     \hspace{-2mm}
%     \begin{minipage}[t]{0.18\textwidth}
%     \includegraphics[width=\textwidth]{rcq_figures/QSIZE_GW_SF_re40}
%     \vspace{-2mm}
%     \end{minipage}
%     \hspace{-2mm}
%      \begin{minipage}[t]{0.18\textwidth}
%         \includegraphics[width=\textwidth]{rcq_figures/QSIZE_GW_NY_re40}
%         \vspace{-2mm}
%         \label{fig:modeling}
%     \end{minipage}
%     \hspace{-2mm}
%     \begin{minipage}[t]{0.18\textwidth}
%         \includegraphics[width=1\textwidth]{rcq_figures/QSIZE_VS_SALT_LAKE_re40}
%         \vspace{-2mm}
%         \label{fig:uniformity}
%     \end{minipage}    
%     \hspace{-2mm}
%     \begin{minipage}[t]{0.18\textwidth}
%     \includegraphics[width=\textwidth]{rcq_figures/QSIZE_VS_LOSANGELES_re40}
%     \vspace{-2mm}
%     \end{minipage}
%     \hspace{-2mm}
%     \label{fig:hotspot4sq}
%     \caption{Varying Spatial Range size experiments at $\varepsilon=0.2$}
% \end{figure*}



% \begin{figure*}[t]
%     \centering
%     \vspace{-10mm}
%     \subfloat{
%     \includegraphics[height=2.5cm]{gmm/conv_vae_recon_7_gmm0.35.png}}

%     \subfloat{
%     \includegraphics[height=2.5cm]{gmm/conv_vae_recon_7_gmm0.55.png}    }
    
%     \subfloat{
%     \includegraphics[height=2.5cm]{gmm/conv_vae_recon_7_gmm0.65.png}    }
    
%     \subfloat{
%     \includegraphics[height=2.5cm]{gmm/conv_vae_recon_7_gmm0.95.png}    }
%     \caption{Gaussian Mixture Model visualization at $\sigma$ varying from 3(top), 5, 7, 9(bottom)}
%         \label{fig: timeline}
% \end{figure*}


==> Spatiotemporal data release (1)/intro.tex <==

\if 0
\begin{itemize}
    \item Location data overtime is useful
    \item No work studied spatiotemporal data release
    \begin{itemize}
        \item 2d or high-d doesn't work well
        \item Companies release data with simple methods and poor privacy accounting
    \end{itemize}
    \item Challenges/opportunities specific to spatiotemporal location data:
    \begin{itemize}
        \item No workload: methods like SNH/DAWA do poorly
        \item Privacy analysis: Users contribute multiple points over time
        \item Existence of temporal patterns
        \item Learned method with new data is hard (snh requires learning for every snapshot)
    \end{itemize}
    \item Contributions
    \begin{itemize}
        \item First method for spatio-temporal location data, user level privacy. This is not true.... Identity is a 
        \item Learned denoising paradigm? Beneficial because it also works on new data, as opposed to SNH?
        \item Novel formulation of problem as "image feature extraction" and use of convolutional filters and variational auto-encoders
        \item Denoising effect is novel in the setting of Differential privacy as it is an unsupervised task.
        % Convolution Filters learn spatial patterns that are both slowly varying and also corrupted by random DP noise. In this instance we show that a Variational AutoEncoder can replace each data point by an approximate local average of surrounding regions. Since nearby points measure very nearly the same underlying value, averaging can reduce the level of noise without biasing much the value obtained.
        \item Variational AutoEncoders offer training regularization to smooth noise as opposed to Autoencoders which simply memorize.
        \item Novel user-level up-sampling method
        \item Extensive experiments with range count/hot spot and forecasting queries
    \end{itemize}
\end{itemize}
\fi

%Mobile apps make extensive use of individual location data to customize user experience. In the process, service providers gather huge amounts of spatio-temporal user traces, which can be highly beneficial in healthcare, transportation and environmental research. 
Several ``data-for-good'' projects \cite{aktay2020google, dataforgood, safegraph_patterns} initiated by major companies (e.g., Meta, Google) release to the public spatio-temporal datasets to benefit COVID-19 spread modeling~\cite{chang2021mobility,rambhatla2022toward, zeighami2021estimating} and understand human mobility \cite{bassolas2019hierarchical, fatehkia2020relative}. Most often, spatio-temporal data are provided in the form of snapshot high resolution population density information, where the released statistics capture population counts in small areas for short time periods. Since high resolution is required for utility (e.g., in modeling COVID hotspots) privacy risks are elevated. To prevent malicious actors from using the data to infer sensitive details about individuals, the released datasets must be first sanitized. Typically, ~\cite{aktay2020google, censusgovKDD18, dataforgood, safegraph_patterns}, {\em differential privacy (DP)} is employed as protection model, due to its formal  protection guarantees that prevent an adversary to learn whether a particular individual's data has been included in the release or not.


Most existing work on DP-compliant publication of location data focused on \textit{single snapshot} releases, where each individual contributes a {\em single location report} ({\em event-level} privacy)~\cite{zhang2017privbayes, xiao2012dpcube, mckenna2018optimizing, hay2009boosting, qardaji2013differentially, cormode2012differentially, zhang2016privtree, li2014data, acs2012differentially, qardaji2013understanding}. When releasing \textit{multiple} snapshots, the ability of an adversary to breach privacy increases significantly, and a shift to {\em user-level} privacy~\cite{dwork2008differential} is required. To protect privacy in this scenario, an increased amount of noise is needed, which often grows linearly in the number of user contributions. Only a handful of techniques~\cite{acs2014case,hien-tmc} considered spatio-temporal location data releases, and their accuracy is subpar. 
%The prefix-tree approach from~\cite{rchen-KDD} was the first to tackle this problem, and built a hierarchical structure that indexes all possible trajectories of users in a discrete location space. Each tree node contains the DP-sanitized count of trajectories that start with a prefix equal to that node's path from the tree root. The follow-up work in~\cite{rchen-ccs} improved accuracy by tabulating noisy counts of all possible sets of n-grams that may belong to a trajectory, not necessarily from its start. However, this approach is still unable to preserve accuracy for n-grams longer than 4-5. Finally, the work in~\cite{hien-tmc} operates a transformation of the trajectory data to a Fourier transform space, and performs sanitization on the Fourier coefficients. This approach's accuracy depends a lot on the type of queries performed, and also fails to preserve data utility beyond several time snapshots.

%Although already done in the industry, to the best of our knowledge, high resolution DP spatiotemporal density release has not been studied in an academic context. Existing work either studies release of spatial data [XXX], temporal data [XXX] or generic high-dimensional data [XXX]. None of the work caters to the specific spatial \textit{and} temporal properties of spatiotemporal datasets, and straightforward generalization of approaches for spatial or temporal data or merely applying high-dimensional approaches to spatiotemporal data yields poor results. 
% \textbf{WE SHOULD MAKE THE BOLD CLAIM THAT WE ARE THE FIRST IN HIGH RESOLUTION SPATIO TEMPORAL DATA RELEASE. CURRENTLY IT SEEMS THE FOCUS IS MORE ON USER LEVEL PRIVACY. \textcolor{red}{GG: THAT CLAIM IS NOT TRUE.}}


%In the absence of approaches for high resolution spatio-temporal data release,
Existing industry projects use simple DP mechanisms that 
%add noise to the population density information without taking 
do not account for specific dataset characteristics \cite{aktay2020google, dataforgood, safegraph_patterns, bassolas2019hierarchical, houssiau2022difficulty}. The amount of privacy budget spent for such data releases is often not reported, or it is excessive~\cite{bassolas2019hierarchical, houssiau2022difficulty, censusgovKDD18}, thus providing insufficient protection.
%to unreasonably large privacy budgets, 
Reports of incorrect privacy accounting in such releases~\cite{bassolas2019hierarchical, houssiau2022difficulty} 
%(or in the industry as a whole [XXX]) 
further necessitate a thorough end-to-end study of custom DP algorithms for spatio-temporal data.

%Temporality complicates location density release, since it requires moving from \textit{event-level} privacy to \textit{user-level} privacy. Research on DP location density publication has so far focused on releasing only spatial information and with {\em event-level} privacy (i.e., each individual contributes a single location report) \cite{zhang2017privbayes, xiao2012dpcube, mckenna2018optimizing, hay2009boosting, qardaji2013differentially, cormode2012differentially, zhang2016privtree, li2014data, acs2012differentially, qardaji2013understanding}. In the case of spatiotemporal data, users contribute multiple location reports over time, which necessitates a shift to {\em user-level} privacy~\cite{dwork2008differential}. In this setting, to release spatiotemporal density information, noise needs to be added to the data whose scale increases proportionately to the maximum number of locations signals contributed by a user, which can be very large in real-world location datasets. Thus, a mechanism that simply adds noise to the density information, as done in the industry \cite{aktay2020google, dataforgood, safegraph_patterns, bassolas2019hierarchical, houssiau2022difficulty}, provides inaccurate density information unless the privacy budget is very large. 

% \begin{figure*}[htb!]
% \begin{center}
% \includegraphics[scale=0.75]{other_figures/system_model_vae.pdf}
% \end{center}
% \caption{Neural Inference For Differentially Private Spatio-temporal Database System}
% \label{fig:system_model}
% \vspace{-1mm}
% \end{figure*}

%To release spatiotemporal density, a privacy preserving mechanism is needed that adds as little noise as possible and is able to preserve density information when noise is added. 
Two key aspects must be addressed. First, one needs to bound {\em sensitivity} (see Section 2 for a formal definition) by limiting the number of location reports from any single user, which can be achieved through sampling.  Density information must be adjusted to account for the fact that it is calculated on a subset of the actual data. Second, the effect of noise added by DP mechanisms must be addressed. Such mechanisms consider the worst-case scenario over all possible data distributions and query configurations, and err on the safe side, adding more noise than strictly necessary. A {\em denoising} post-processing step that leverages spatio-temporal data characteristics can significantly boost accuracy, while still satisfying privacy. Recent advances in neural networks, such as variational auto-encoders (VAE), are good at capturing complex density patterns, and can enable effective denoising.
%We draw on new approaches in the machine learning literature [XXX] that show neural networks are able to capture patterns in the data from noisy observations. Such approaches train neural networks on non-noisy observations and show that when making inferences, a neural network can accurate capture the patterns even if the input is noisy. With differential privacy, the situation is more challenging, because  training needs to be done on noisy observations as well. Furthermore, to be able to utilize machine learning effectively in our setting, modeling choices and learning techniques have to be hand-crafted for the specific problem of spatiotemporal data release to be able to learn the characteristics of such datasets. 

%Recently, a new line of research [XXX] has focused on reducing the impact of noise through machine learning after the noise is added to the data. Intuitively, such approaches utilize repeating patterns in the data to capture the data distribution. By allowing machine learning models to capture the patterns from noisy observations, a model is learned that represents the data better than the noisy version. However, 

%There are two ways to reduce the noise impact. (1) As is traditionally done in the location density release literature [XX], density information is released at resolutions (which are potentially different for different parts of the space) that achieve good signal-to-noise ratio. Such approaches create a partitioning of the space that is finer where the data is estimated to be dense and coarser otherwise. However, such density estimates are often inaccurate and requires spending privacy budget to compute. Second, if the desired density information is at a higher resolution than provided by DP mechanism, the answer is uniformly divided based on the covered area. This introduces extra error, as spatial datasets often exhibit large skewness. (2) On the other hand, 


We propose {\em VAE-based Density Release} (\name{}), a system specifically designed for accurate, DP-compliant release of spatio-temporal data.
%for  accurate DP release of high resolution spatiotemporal location density. 
% A core feature of \name{} (illustrated in Fig.~\ref{fig:system_model}) 
Noisy spatio-temporal data histograms exhibit patterns akin to visual patterns in image sequences. This observation allows one to leverage a vast amount of work on image pattern recognition and apply it to spatio-temporal data. \name{} sanitizes density information by adding DP-compliant noise, then improves  accuracy by performing a post-processing {\em denoising} step based on convolutional neural networks (CNN). We utilize {\em variational auto-encoders (VAE)} to capture data patterns without fitting to the noise. We employ multi-resolution learning to capture patterns at multiple granularities, improving accuracy for a broad range of query extents.

To reduce sensitivity of user-level privacy, we reduce the number of input samples from any individual in a DP-compliant way. To counter-balance the effect of sampling, we design a novel private statistical estimator which scales up query results to preserve accuracy. This permits us to control the sensitivity in user-level privacy without significantly affecting accuracy.

%is by aggregating parts of the space, answering queries on the aggregate with differential privacy, and uniformly splitting the answer across the sub partitions of the space. The problem is that the aggregation is done manually and uniformity assumption doens't hold on the places that are close to each other. However, repeating patterns can exist, and aggregating answers across these patterns can help improve the accuracy. CNN can help find/aggregate those patterns. 
%External informaion, posterior, 

%This is exacerbated by the fact that existing mechanisms (e.g., Laplace, geometric, Gaussian) add more noise than strictly necessary to the query results, compromising accuracy. A privacy mechanism must consider the worst-case scenario over all possible data distributions and query configurations, and protect against that case. Since in-depth characterization of data and query placement is difficult, privacy mechanisms err on the safe side, and add more noise than necessary. This problem is amplified when shifting to user-level privacy by the fact that, in the worst case, sensitivity grows linearly with the maximum count of location reports among all users.


%The main challenge in incorporating temporality in location data release is moving from \textit{event-level} privacy to \textit{user-level} privacy. So far, research on DP location density publication has focused on releasing only spatial information and with {\em event-level} privacy (i.e., each individual contributes a single location report) \cite{zhang2017privbayes, xiao2012dpcube, mckenna2018optimizing, hay2009boosting, qardaji2013differentially, cormode2012differentially, zhang2016privtree, li2014data, acs2012differentially, qardaji2013understanding}. In the case of spatiotemporal data, users contribute multiple location reports over time, which necessitates a shift to {\em user-level} privacy~\cite{dwork2008differential}. In this setting, to release spatiotemporal density information, noise needs to be added to the data whose scale increases proportionately to the maximum number of locations signals contributed by a user, which can be very large in real-world location datasets. Thus, a mechanism that simply adds noise to the data, such as [XXXXX], provides inaccurate density information unless the privacy budget is very large. This is exacerbated by the fact that existing mechanisms (e.g., Laplace, geometric, Gaussian) add more noise than strictly necessary to the query results, compromising accuracy. A privacy mechanism must consider the worst-case scenario over all possible data distributions and query configurations, and protect against that case. Since in-depth characterization of data and query placement is difficult, privacy mechanisms err on the safe side, and add more noise than necessary. This problem is amplified when shifting to user-level privacy by the fact that, in the worst case, sensitivity grows linearly with the maximum count of location reports among all users.


%Nonetheless, exploiting temporality can help improve the accuracy. For example, population density for a particular place may repeat over time, so by carefully utilizing the temporal dimensions, one can obtain more information about locations in the city that can help better estimate population density over time. 


\if 0
Mobile apps make extensive use of individual location data to create customized user profiles and to improve service quality of their customers. In the process, service providers gather huge amounts of location data, which can be highly beneficial in healthcare, transportation and environmental research. Several ``data-for-good'' projects have been initiated by major companies (e.g., Meta, Google) that release such data to the public, after performing sanitization. Data sanitization prevents malicious entities from using location data to infer sensitive details about individuals. Typically, the de-facto standard of {\em differential privacy (DP)} is employed as protection model, due to its formal statistical protection guarantees that limit the ability of an adversary to learn whether a particular individual's data has been included in the release or not.

Most work in the area of DP-compliant publication of location data has focused on releasing single snapshots, where each individual contributes a single location report~\cite{zhang2017privbayes, xiao2012dpcube, mckenna2018optimizing, hay2009boosting, qardaji2013differentially, cormode2012differentially, zhang2016privtree, li2014data, acs2012differentially, qardaji2013understanding}. This setting is referred to as {\em event-level} privacy. In the case of trajectory data, each individual contributes multiple reports, which is a significant complicating factor,  as it requires a shift to {\em user-level} privacy~\cite{dwork2008differential}, which in turn increases the noise level that must be added to achieve protection. Only a handful of techniques have addressed private trajectory release, and none of them is able to preserve data accuracy beyond trajectory lengths of 4-5 snapshots. The prefix-tree approach proposed in~\cite{rchen-KDD} was the first to tackle this problem, and builds a hierarchical structure that indexes all possible trajectories of users in a discrete location space (the authors consider a finite set of logical locations consisting of the subway stops in Montreal, Canada). Each tree node contains the DP-sanitized count of trajectories that start with the prefix equal to that node's path from the tree root. The follow-up work in~\cite{rchen-ccs} improved accuracy by tabulating noisy counts of all possible sets of n-grams that may belong to a trajectory, not necessarily from its start. However, this approach is still unable to preserve accuracy for n-grams longer than 4-5. Finally, the work in~\cite{hien-tmc} operates a transformation of the trajectory data to a Fourier transform space, and performs sanitization on the Fourier coefficients. This approach's accuracy depends a lot on the type of queries performed, and also fails to preserve data utility beyond several time snapshots.

There are two main reasons that cause poor accuracy for trajectory santization approaches: the use of blunt sanitization mechanisms, and the increase in sensitivity when shifting from event-level to user-level privacy. A privacy mechanism must consider the worst-case scenario over all possible data distributions and query configurations, and protect against that case. Since in-depth characterization of data and query placement is difficult, existing mechanisms (e.g., Laplace, geometric, Gaussian) err on the safe side, and add more noise than strictly necessary to the query results, compromising accuracy. This problem is amplified when shifting to user-level privacy by the fact that, in the worst case, sensitivity grows linearly with the maximum count of location reports among all users.

We propose a set of techniques that directly tackle this problems. First, we introduce a neural network-based approach to improving accuracy by performing an advanced post-processing step which offsets the negative effects of DP-added noise. According to differential privacy theory~\cite{?}, any post-processing step is safe, in the sense that the privacy requirement will still be preserved. On the other hand, clever post-processing techniques can reduce the amount of noise introduced by generic mechanisms, and bring it closer to the minimum theoretical amount required to achieve protection. We refer to this process as {\em denoising}. Our proposed denoising technique relies on variational auto-encoders to capture subtle patterns specific to location datasets, and is able to significantly boost accuracy. We also employ multi-resolution learning, in order to capture location data patterns at multiple granularities, and thus improving accuracy for a broad range of query extents.

Second, we devise a comprehensive strategy to reduce sensitivity of user-level privacy through sampling. We reduce the number of input samples from any particular individual in a way that preserves DP, while at the same time preserves movement accuracy, without compromising trajectory characteristics. We design a novel approach that uses a DP-compliant statistical estimator to derive the count of location reports that must be preserved to obtain a good sensitivity-accuracy trade-off. This allows us to tightly control the sensitivity of user-level privacy without significantly affecting trajectory information.
\fi





Our specific contributions are:
\begin{itemize}
    \item We propose an end-to-end privacy-preserving system for spatio-temporal datasets that satisfies user-level differential privacy and preserves data accuracy;
    \item We introduce a novel approach to user-level sampling that reduces sensitivity while preserving density information across time;
    \item We design a novel denoising technique that uses variational auto-encoders and image feature extraction concepts to accurately model patterns in spatio-temporal data;
    \item We design a technique to offset the effects of location sampling in order to provide accurate query answers; to that extent, we employ DP-compliant statistical estimators;
    \item We perform an extensive experimental evaluation on real data which shows that the proposed approach clearly outperforms all existing approaches.
\end{itemize}

 We provide background information and formulate the studied problem in Section 2. Section 3 introduces the proposed sampling and denoising techniques. Section 4 explores system design trade-offs. Section 5 presents the experimental evaluation results. We survey related work in Section 6 and conclude in Section 7.   

==> Spatiotemporal data release (1)/learned_denoising.tex <==
%We start by presenting \textit{learned denoising}, a core component of our method, in a simplified setting. In this section, we only consider DP release of spatial data. This is, in fact, a typical setting considered in many related work [XXX]. We then present our method for spatiotemporal data in Sec.~X, where we utilize learned denoising to provide accurate answers. We first present the concept of learned denoising in Sec.~\ref{sec:spatial:learned_denoising} and present a complete algorithm for spatial data release utilizing learned denoising in Sec.~\ref{sec:spatial:algo}.

%\subsection{Learned Denoising for Spatial Data}\label{sec:spatial:learned_denoising}

%\subsubsection{Setup} 
%In spatial data release, we are given an $m\times m$ histogram, $H$, represented by a 2d array where each cell in the array corresponds to the number of location signals in the particular cell. The goal is to publish $H$ while preserving differential privacy. Most methods, with a few exceptions [SNH, XX], aggregate cells in the histogram and add noise to the cells to obtain a noisy version of $H$, $\bar{H}$. We can assume $\bar{H}$ is also an $m\times m$ histogram (or otherwise uniformity assumption can be used to obtain the desired granularity). This setup is the common implementation of DP algorithm in various system XXX, where algorithms take an $m\times m$ histogram, $H$ as input and output another $m\times m$ histogram, $\bar{H}$, which is a noisy version of $H$. 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{illustrations/data_collection.pdf}
    \caption{(a) and (b): real-world complete and sampled dataset of location reports over time in Houston. (c) and (d): exact and noisy 3-d histograms created from the sampled dataset, higher brightness shows higher density.}
    \label{fig:data_collection}
\end{figure}

\begin{comment}
\begin{figure}
    \centering
    \begin{minipage}[t]{0.46\linewidth}
        \includegraphics[width=\textwidth]{other_figures/datasize_vs_sampled.eps}
    \end{minipage} 
    \hfill
    \begin{minipage}[t]{0.46\linewidth}
    \includegraphics[width=\textwidth]{other_figures/hist_signals_per_user.eps}
    \end{minipage}
    \caption{Veraset Houston Data Statistics}
    \label{fig:stats}
\end{figure}
\end{comment}



\subsection{Data Collection}\label{sub:collection}
Data collection uses a combination of sampling and noise addition to create a differentially private histogram of the data without making any modelling assumptions. In the case of spatio-temporal data, simple noise addition will lead to poor quality results, as the amount of noise needed will destroy any meaningful signal in the data. We first discuss the naive solution and its specific challenge for spatiotemporal data; subsequently, we show how sampling is able to improve the accuracy; finally we present the details of the data collection mechanism. We use as running example a real world dataset of location reports from Houston, TX, USA (see Section \ref{sec:exp} for exact details of dataset). %This dataset is shown in Fig.~\ref{fig:data_collection} (a). 

\textbf{DP Histogram Release}. Given dataset $D$  with location reports from different users over time, the goal is to create a histogram of the data while preserving $\varepsilon$-DP. One way to do this (without making any modeling assumptions) is to first create the true histogram of the data $H$, and then add independent Laplace noise, $Lap(\frac{\Delta}{\varepsilon})$ to each cell of the histogram, where $\Delta$ is the sensitivity of the query of number of data points falling inside a cell. This sensitivity is equal to the maximum number of points, $k_{\max}$, a user contributes to the dataset. Thus, the DP histogram of the data can be written as $\bar{H}=H+Lap(\frac{k_{\max}}{\varepsilon})$, where independently generated random noise is added to each cell of the histogram.

\textbf{Challenge for Spatiotemporal Histograms}. %In spatiotemporal datasets, the number of data points contributed to the dataset by each user varies significantly across users. While most users contribute few points, some prolific users may contribute a very large number of points. In fact, the number of points a user contributes often follows a power law \cite{muchnik2013origins, yang2015nationtelescope}. For our running example Houston dataset, the maximum number of points contributed by a user is $k_{\max}=90,676$ (in real datasets, location updates from mobile apps reporting user movements often leads to large number of contributions, with the amount of user contributions varying due to different app utilization across users). %At the same time, for most spatial and temporal ranges of practical interest, the number of location signals at that data point is much less than 4000XXX. 
\revision{As discussed in Sec.~\ref{sec:data_model}, real-world location datasets follow power law distribution. For the Houston dataset, $k_{max}=90,676$, while 80\%  of users have at most 100 points. In this dataset, for ranges of 30 meters and 1 hour time periods, only 1 percent of the histogram cells have values more than 25. In such datasets, applying the above DP histogram method, without adjusting for the power law distribution across users, leads to poor accuracy. In our running example,} Laplace noise scaled to $k_{\max}/\varepsilon$, for any reasonable value of $\varepsilon$, wipes out any meaningful information in all but a few cells.

\textbf{Sampling to Bound Sensitivity}. Instead of using all the data points of users when creating the histogram, we sample a maximum of ${k}$ points per user, for a user parameter ${k} < k_{\max}$. Specifically, we sample a subset of points $D_s \subseteq D$ as follows: for any user with more than ${k}$ points, we sample ${k}$ of their points uniformly at random. For users with at most ${k}$ points, we keep all their points. This reduces the sensitivity of releasing histogram to ${k}$, requiring that we add only noise $Lap(\frac{{k}}{\epsilon})$ to each cell of the histogram. In this way, we can exploit the skewness in user contributions to the dataset, because by setting ${k}$ to a small value, we are able to retain most of the original data. For the Houston dataset, setting ${k}$ to 128 captures nearly 25\% percent of the data, while reducing sensitivity by 700\%. Consequently, we bias the data distribution in order to reduce variance in query reporting. Nonetheless, sampling introduces \textit{sampling error} in the answers over  histogram  $D_s$. In our statistical refinement step (Sec.~\ref{sub:refinement}), we discuss how we can counter this source of error. We further discuss trade-offs arising in our method based on the choice of $k$ in Sec.~\ref{subsec:system}.

%{\tt GG: this is overly-simplistic, we need a more in-depth discussion on how is this threshold chosen, why is that a good setting, then have some pseucocode/formula showing how to determine it.}

%The interplay between sampling error and noise is data dependent. Fig.~\ref{fig:sampling} shows this interplay at various sampling levels for our running example, which shows that sampling too few or too many points is detrimental. I DON"T THINK WE NEED THIS HERE CUASE IT RAISES QUESTION ON HOW TO SET $k$, MAYBE WE CAN HAVE IT IN THE EXPS for various datasets and say it doesnt matter.  

% By setting $\hat{k}$ to a small value, one can obtain most of the original dataset and the benefits of increasing $\hat{k}$ diminishes since adding more points per user does not increase the total number of points sampled significantly, as shown in Fig.~\ref{fig:sampling}.

%\textbf{Final Mechanism}.
\textbf{Summary and Example}. Data collection is depicted in Fig.~\ref{fig:data_collection} for our running example, where we release a noisy $50$$\times$$50$$\times50$ histogram of the dataset of location reports in Houston (\revision{granularity chosen for better visualization}). We sample up to ${k}$ for each user from the complete dataset $D$ to create the sampled dataset $D_s$. Then, we create a 3-dimensional histogram, $H_s$ of $D_s$. Finally, we create the histogram $\bar{H}=H_s+Lap(\frac{{k}}{\varepsilon})$ so that the data collection process satisfies $\varepsilon$-DP. The output of the data collection step is the noisy histogram $\bar{H}$. The output in Fig.~\ref{fig:data_collection} (d) shows the noisy histogram, where each cell corresponds to noisy density in a 800$\times$800 meter cell for a 4 hour time period. 



\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{illustrations/spatial_pattern_over_time.pdf}
    \caption{Spatial patterns over time on histogram slices}
    \label{fig:histogram_overtime}
\end{figure}

\if 0

\begin{figure}
    \centering
    \includegraphics[width=0.32\columnwidth]{illustrations/heat_H214.png}
    \includegraphics[width=0.32\columnwidth]{illustrations/heat_H215.png}
    \includegraphics[width=0.32\columnwidth]{illustrations/heat_H216.png}
    \caption{Houston Histogram over time}
    \label{fig:histogram_overtime}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.32\columnwidth]{illustrations/56_heat_HN0.png}
    \includegraphics[width=0.32\columnwidth]{illustrations/56_heat_HN1.png}
    \includegraphics[width=0.32\columnwidth]{illustrations/56_heat_HN2.png}
    \caption{Houston Histogram over time, coarse}
    \label{fig:histogram_overtime_coarse}
\end{figure}
\fi


\subsection{Learned Denoising}\label{sub:denoising}
Denoising uses machine learning, specifically VAEs, to identify spatial-temporal patterns, and  utilizes them to improve histogram accuracy. Our main observations are: (1) spatio-temporal histograms are similar in nature to a sequence of images, thus methods from image representation learning can be applied to capture data patterns; (2) regularized representation learning can ensure the model learns a denoised representation of the data while not over-fitting noise; and (3) multi-resolution learning can capture spatio-temporal patterns at different granularities. %We first detail these observations and then present the complete denoising algorithm.

\subsubsection{Design Principles\nopunct}\hfill\\
%The following observations form the basis of our learned denoising algorithm.

\textbf{Denoising with Regularized Representation Learning}. We want to derive a denoised histogram $\hat{H}$ from $\bar{H}$ that is similar to $H$, where similarity is measured as norm $\lVert H-\hat{H}\rVert$, i.e., the sum of squared differences across all cells of the histograms. To achieve this, consider a function {\tt encoder}($\bar{H}$) that creates an encoding, $z$, of the noisy histogram, and a function {\tt decoder}($z$), that outputs a histogram, $\hat{H}$, from the encoding $z$. Consider the problem of learning an encoding $z$ (i.e., by learning functions {\tt encoder}(.) and {\tt decoder}(.)), so that $\lVert\hat{H}-\bar{H}\rVert$ is minimized, where we call $\lVert\hat{H}-\bar{H}\rVert$ the {\em reconstruction error}.
%In the absence of any constraints on $z$, reconstruction error can be easily made to be zero, by setting encoder and decoder to identity functions, so that $z$ and $\hat{H}$ become the same as the input histogram, $\bar{H}$. 
%However, we do not want an exact representation because $\bar{H}$ is noisy, 
Our goal is to obtain an encoding $z$ that summarizes the patterns in $\bar{H}$, since such patterns will also exist in the true histogram $H$. 
%By enforcing constraints on $z$, we can learn an encoding that does not represent exactly $\bar{\H$, but captures it succinctly by learning repeating patterns. 
To see why this is possible, observe that a constraint on $z$ limits its representation power. For instance, by setting the dimensionality of $z$ to be lower than that of $\bar{H}$, $z$ cannot contain as much information as $\bar{H}$. Thus, a regularized encoding, $z$, that minimizes the reconstruction error cannot contain all the information in $\bar{H}$. By learning a regularized representation, $z$, a model is able to capture the patterns in $\bar{H}$ that best summarize the histogram. Such a summary \revision{will be less noisy}, as \revision{noise} does not generalize across the histogram (noise is independently added to each cell) and can only be memorized individually per cell. Thus, by properly regularizing the encoding, we can find an encoding that is denoised, i.e., contains the patterns in the data, but \revision{less} noise. Subsequently, by decoding such a representation, we can obtain a denoised histogram. That is, the regularization ensures that even though we try to minimize the reconstruction error $\lVert\hat{H}-\bar{H}\rVert$, we obtain a histogram such that $\lVert\hat{H}-{H}\rVert$ is smaller than $\lVert\bar{H}-{H}\rVert$.


\textbf{Spatial Patterns as Visual Patterns}. Denoising with regularized representation learning will be beneficial only if the model is able to extract the patterns in the histogram. To facilitate this, we observe that a 3-d histogram of the data can be seen as a sequence of images, as shown in Fig.~\ref{fig:histogram_overtime} for our running example. The left side of Fig.~\ref{fig:histogram_overtime} plots the 3-d histogram which represents a time-series of two-dimensional histograms, one per each timestamp. We call each of these 2-d histograms a \textit{slice}. On the right side of the figure, we plotted various slices, each corresponding to a different timestamp. We can see that spatial patterns in the histogram are in fact visual patterns. For instance, patterns corresponding to roads or busy areas can be seen as lines or blobs in the image. \revision{In real world location datasets, we expect such consistent patterns across space that may also be repeating over time (see Sec.~\ref{sec:data_model} regarding location data characteristics)}, suggesting that representation learning can be achieved effectively using techniques from image feature learning. 

\begin{comment}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{illustrations/spatial_pattern_over_granularities.png}
    \caption{A histogram slice with varying coarseness}
    \label{fig:histogram_overtime_coarse}
\end{figure}
\end{comment}

\textbf{Multi-Resolution Learning (MRL) at Varying Granularity}. Spatial patterns in the data exist at various granularities of the input histogram. %Fig.~\ref{fig:histogram_overtime_coarse} illustrates several degrees of histogram resolution, from finest (left) to coarsest (right). We observe that 
Patterns at finer resolutions feature roads more prominently, while patterns at coarser granularities feature primarily neighbourhood densities. Furthermore, the patterns in coarser granularity histograms are less affected by noise, which allows the model to still infer spatial density. We propose to train a single model based on data configured at multiple granularities to improve denoising accuracy. 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{illustrations/training_preperation.pdf}
    \caption{Training set preparation}
    \label{fig:learned_denoising_prep}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{illustrations/Learned_Denoising.pdf}
    \caption{Model Training}
    \label{fig:learned_denoising}
\end{figure}


\subsubsection{Denoising with Convolutional VAEs}\label{sec:decnoising_detail}
Based on the above principles, we utilize convolutional VAEs to denoise the histogram $\bar{H}$. We first provide an overview of our algorithm, then provide more details on the role of regularization in our methodology, and finally present the algorithm pseudocode.

%\textbf{Overview}. 
Our method consists of three stages: (1) training data preparation, (2) model training and (3) model inference. We discuss each below. 

\textit{Training data preparation}. Recall that we are given a noisy 3-d histogram, $\bar{H}$, where the 2-d histograms resulting from each slice contain density information for different locations. Thus, we view the 3-dimensional histogram $\bar{H}$ as a set of two dimensional histograms, where the $i$-th element in this set, $\bar{H}_i$, is a 2-dimensional slice corresponding to the $i$-th timestamp. This is shown on the left side of Fig.~\ref{fig:learned_denoising_prep}. Then, as shown on the right side of Fig.~\ref{fig:learned_denoising_prep}, to utilize multi-resolution learning, we aggregate each of the slices at various resolutions. For instance, every block of $2 \times 2$ cells in $\bar{H}_i$ are aggregated to obtain a new 2-d histogram which has a coarser granularity. This aggregation is done at $r$ different resolutions, and all the aggregated histograms are put together in a training set $T$. \revision{We remark that although CNN layers can extract information at multiple resolutions from an input image, multi resolution learning cannot be achieved by adding a CNN layer to the architecture, since doing so would also change the loss function, in order to enforce the information to be captured at multiple resolutions (loss is over all training data i.e., at different resolutions) .}

\textit{Model Training}. We use a convolutional VAE to perform regularized representation learning. An encoder, which is a CNN, takes as input each 2-d slice and outputs a representation for it. Denote by {\tt encoder(.;$\theta_e$)} the network whose parameters are $\theta_e$, and let $\ell$ be the dimensionality of the representation output. The representation is then fed to a decoder, which is another neural network, denoted by {\tt decoder(.;$\theta_d$)}, where $\theta_d$ are the parameters of the decoder. The output of the decoder is a 2-d histogram, as shown in Fig.~\ref{fig:learned_denoising}. To simplify notation, we directly input a set of 2-d histograms to the encoder, in which case the output is also a set of representations (similarly for decoder). The model is trained to minimize a reconstruction loss, which is the difference between input slice and the output slice, and a regularization loss, which ensures that the learned representation follows some regularization constraints. 

\textit{Model Inference}. Each slice, $\bar{H}_i$, is passed through the convolutional VAE, first encoded and then decoded, to obtain the denoised representation for $\bar{H}_i$. This is done for all timestamps, $i$, which allows us to obtain a denoised 3-d histogram, $\hat{{H}}$. Note that, inference is not performed on any aggregated histogram (via multi-resolution), but only on the original noisy histogram $\bar{H}$. In other words, the output of learned denoising is a single 3-d histogram $\hat{{H}}$, which is at the same resolution as the noisy input histogram $\bar{H}$.

\textbf{VAE and Regularization Details}. We discuss parts of the VAE design relevant to the problem of denoising. Further details of our model can be found in Sec.~\ref{sec:exp}.  We utilize the Vector Quantized variant of VAE (VQ-VAE), where the encoding is forced to follow a certain discrete structure \revision{(Sec.~\ref{sec:dicsussion:hyperparams} discusses other possible variants and modelling choices)}. A discrete set, $\Upsilon$, called a \textit{codebook}, of $\mathcal{B}$ different encodings, $\Upsilon=\{e_1, ..., e_{\mathcal{B}}\}$, where each $e_i$ is $\ell$-dimensional, is learned, and VAE training process forces the encoder to output an encoding that is similar to an element in the codebook. Recall that {\tt encoder(.;$\theta_e$)} is a convolutional neural network that takes as input a 2-d histogram. For an input 2-d histogram in our training set, $\bar{T}$, {\tt encoder($\bar{T};\theta_e$)} provides a set of representations $z$. These representations are then input to the decoder to obtain reconstructions $\hat{T}=$ {\tt decoder($z;\theta_d$)}. VQ-VAE defines a distance function between $z$ and $\Upsilon$, $d(z, \Upsilon)$, that measures how similar the encodings are to the codebook. $d(z, \Upsilon)$ is then minimized in the training process to ensure the encoder learns representations that are similar to the codebook. We call $\mathcal{L}_G(z)=d(z, \Upsilon)$ the regularization loss and define $\mathcal{L}_C(\hat{T})=\sum_{i=1}^{|\bar{T}|}\lVert \bar{T}_i-\hat{T}_i\rVert^2$ as the reconstruction loss, where $T_i$ is the $i^{th}$ slice in the training set and $\hat{T}_i$ is the output of the VQ-VAE on the $i^{th}$ training slice. We then train VQ-VAE to minimize $\alpha\times\mathcal{L}_G(z)+\mathcal{L}_C(\hat{T})$, where parameter $\alpha$ is introduced to control the amount of emphasis on the regularization. \revision{We discuss setting the hyperparameters in Sec.~\ref{sec:dicsussion:hyperparams}}.

%as a testament to the benefits of regularized representation learning for DP data denoising and release.  

% As we add more slices to training, learning stabilizes and the the derived patterns achieve better denoising performance. 



%learns a discrete latent space using Vector Quantization (VQ) techniques. VQ-VAE \cite{van2017neural} utilizes a latent embedding space of dimension $[\mathcal{B}, \ell]$ where $\mathcal{B}$ are the number of embeddings and $\ell$ is the dimensionality of each latent embedding vector, i.e. $e_i\in \mathbb{R}^\ell$. The parameter $\mathcal{B}$ controls the bottleneck and thus the ability of the model to fit/over-fit the data. 



%We observe that \textit{Variational Auto-Encoders} (VAEs) \cite{kingma2013auto} are able to learn denoised encodings of the noisy histogram and use the encoding to create histograms that better represent the true data compared with the noisy input. VAEs learn denoised encodings through  whose benefit in our setting can be summarized as follows. (1) VAEs learn a \textit{low-dimensional} encoding of the noisy histogram that is optimized to be able to reconstruct the noisy histogram as accurately as possible. To maximize this accuracy, the low-dimensional encoding can only contain patterns in the histogram that generalize across the cells of the histogram. On the other hand, noise is added independently and at random to each cell, so to accurately reconstruct the noise, the noise has to be memorized for each cell. Since the representation is in a much lower dimension compared with the number of cells in the histogram, this memorization cannot happen. Thus, the dimensionality regularization ensures that the model can only learn the patterns in the histogram. (2) The low dimensional encoding space is regularized to be semantically meaningful. For instance, a random vector in the encoding space (that doesn't correspond to any real input), when decoded resembles a real input. This further forces the model to learn a representation consisting of patterns in the data rather than the noise.  XXXXXX

%CNNs take advantage of the hierarchical pattern in data and assemble patterns of increasing complexity using smaller and simpler patterns embossed in their filters. Simply put, convolutional functions can be applied to capture the spatial patterns in the data as they exploit the local relationships across different parts of the histogram. 


\if 0

\textbf{Overview}. Fig.~\ref{fig:learned_denoising} shows the design of the convolutional VAE used in our setup. The VAE takes as input a noisy two dimensional histogram, $\bar{H}_i$,  visualized as an image. An encoding module uses learned convolutional filters to extract patterns from the data and represent it as a low dimensional vector. The decoder takes the low dimensional vector as an input and construct a histogram $\hat{H}_i$, which is the output of the VAE. 

The model is trained across all the 2-dimensional histograms. To learn patterns at different granularities, we augment the training set with histograms at different graunularities. {\tt [GG: How many granularites, and how are they chosen? Pseudocode/formula?]} We aggregate adjacent cells in the histogram together to obtain coarser histograms, and add the coarse histograms to our training set. The training objective is to minimize a reconstruction loss and an encoding regularization loss. {\tt [GG: Define this loss measure, e.g., equation and show why it is meaningful.]} The first makes sure the reconstructed histogram looks similar to the input histogram, while the second makes sure the encoding space is semantically meaningful. Since the encoding is low dimensional and regularized, the model is forced to utilize patterns in the data for reconstruction, and noise values cannot be contained in the encoding. Thus, the noise is reduced in the reconstructed histogram.
\fi







\textbf{Complete Denoising Algorithm}. The complete denoising process is shown in Alg.~\ref{alg:learned_denoising}. %VAEs create a low dimensional encoding space that follows a prior structure, denoted by $\pi$, and optimize the neural network that encodes the data so that it follows the prior structure while being able to accurately reconstruct the input histogram. $\pi$ can be a prior distribution on the encoding (e.g., Gaussian \cite{kingma2013auto}) or a specific discretized structure \cite{van2017neural}. VAEs define, for a set of encodings, $z$, created by the model, a distance function $d(z, \pi)$, that measures how well the encodings follow this structure. We call this distance function a regularization loss (specifics of $\pi$ and $d$ are defined in our experiments in Sec.~\ref{sec:exp} based on existing VAE literature). We introduce two parameters, $\mathcal{B}$ and $\alpha$, that control the extent of regularization in the VAE. $\mathcal{B}$ is the dimensionality of the encoding space, and regularizes how much information can be represented in the encoding. $\mathcal{B}$ controls the importance of the regularization loss.  Furthermore, the system parameter, $r$, controls how coarse the histogram with maximum coarsness should be.
Lines~\ref{alg:denoise:create_train}-\ref{alg:denoise:augment} show how the training set is augmented with histograms at varying granularities.  Lines~\ref{alg:denoise:enc}-\ref{alg:denoise:dec} create a CNN as an encoder and a Transposed CNN as the decoder. The model is trained in Lines~\ref{alg:denoise:train_begin}-\ref{alg:denoise:train_end}, where at Line~\ref{alg:denoise:encode} the encoder outputs encodings of the histograms in the training set and the encodings are then decoded by the decoder to reconstruct the histograms in Line~\ref{alg:denoise:decode}. The model is then optimized with stochastic gradient descent to minimize the reconstruction loss and the regularization loss. %The reconstruction loss, $\lVert \bar{T}_i-\hat{T}\rVert^2$ is the squared distance between the values in each cell predicted by the decoder and the input. 
Finally, after convergence, a forward pass of the model yields the denoised histogram. 

We have kept the discussion of convolutional VAEs at a high level and only provided details for ideas that pertain to the problem of denoising, without discussing in-depth the technical details in VAE and VQ-VAE design such as commitment and alignment loss \cite{wu2020vector}, the reparametrization trick \cite{xu2019variance} and their relation to regularization. We provide implementation specific details of VQ-VAE in Sec.~\ref{sec:exp}.

\revision{\subsubsection{\revision{Modelling and Hyperparameter choice}\nopunct}\label{sec:dicsussion:hyperparams}\hfill\\
\revision{\textbf{VAE Type and Architecture}. VAE architectures model data distribution over continuous (e.g., in Gaussian-Process VAE) or discrete (e.g., Vector-Quantized VAE) latent space variables. We limit our discussions to the discrete variant, even though either of these architectures are effective for use in VDR. The regularized representation learning ability of VAEs is essential to VDR, but we do not expect the specific distribution enforced on the latent variables to significantly impact accuracy. Our choice of VQ-VAE is due to its faster training time and convergence rate compared with other variants (see Fig. \ref{fig:gpvae_vs_vqvae} in Sec. \ref{subsec:settings}). Lastly, since we focus on location data that, as discussed in Sec. \ref{sec:data_model}, show homogeneous characteristics across datasets, our choice of VAE architecture is not sensitive to the specific data subset. Thus, we utilize VQ-VAE exactly as in \cite{razavi2019generating} without any modification and across all datasets.} } 

\revision{\textbf{Regularization Parameters}.}
Parameters $\mathcal{B}$ and $\alpha$ control how regularization benefits denoising. (1) $\mathcal{B}$ controls the representation power of the encoding space: the smaller $\mathcal{B}$ is, the less information can be captured by different encodings, as the encodings for different slices are forced to be similar. On the other hand, when $\mathcal{B}$ is large, different slices are allowed to take different representations, as the codebook allows for more variability.  (2) $\alpha$ controls how much the encoder is forced to adhere to the codebook. When $\alpha$ is small, the encoder can learn representations that do not follow the discretized structure. It allows learning different encodings for different slices, thus memorizing the information within slices instead of learning patterns that generalize. 

We find significant benefit in invoking both of the above regularization aspects of VQ-VAEs. Specifically, we saw worse performance when setting $\alpha$ to a small value, confirming our regularized learning design principle and emphasizing the need for regularizing the encoding space. Denoising ability also suffers when $\mathcal{B}$ is too small or too large; the former because not enough information can be stored in the learned encoding, and the latter because the encoding can become noisy (due to insufficient regularization). \revision{Since we focus on location data that, as discussed in Sec. \ref{sec:data_model}, show homogeneous characteristics across datasets, our choice of regularization parameters is not sensitive to the specific data subset. As such, we fixed $\alpha=1$ and $\beta=128$ across all datasets in our experiments.}   %Furthermore, privacy budget affects the extent of regularization required. For instance, when privacy budget is large, noise of smaller magnitude is added and thus finer grained patterns are preserved in the data. By increasing $\mathcal{B}$ in such a scenario, the model can learn more detailed features of the data. On the other hand, for smaller privacy budgets, $\mathcal{B}$ needs to be small so that the model does not overfit the noise. We further investigate these trade-offs in Sec.~\ref{sec:exp}.

\subsection{Statistical Refinement}\label{sub:refinement}
Given that the values in the denoised histogram are based on the sampled dataset, they will be an underestimation of the true counts. In this section, we study how the values can be scaled to accurately represent the true counts. We first discuss how differential privacy complicates this process of statistical refinement, then present notations and assumptions in our method and finally discuss the statistical refinement step.

\subsubsection{Estimation with Differential Privacy}\label{sec:refine:challanges} Recall that we sampled a dataset $D_s$ from the true dataset $D$, and created a noisy histogram $\bar{H}$ from the sampled set. We retained up to $k$ points per user, hence the size of $D_s$ is smaller than $D$. Thus, the number of data points that fall inside the histogram created based on $D_s$ will be an underestimation of the true number of data points. To adjust the observed answers based on sampled data points we need to scale them, so that they accurately represent the true numbers. However, DP affects how this scaling can be done.

\textbf{Noisy Observations}. 
%Since we have access only to the noisy histogram $\bar{H}$ and not the observed histogram $H$. 
Scaling the values in $\bar{H}$ scales both the added noise and the observed values, thus amplifying the random noise. In other words, by scaling the observed values, we reduce the bias in our estimation (i.e., account for underestimation), but this scaling increases the variance in our estimation because the random noise gets amplified. Thus, in the case of sampling with differential privacy, it is important for our method to account for both bias and variance in the estimation.

\textbf{Private Sampling Procedure}. The sampling procedure is data dependent, and its specific details may be unknown, due to privacy requirements. Therefore, we aim to derive a refinement approach that is agnostic to the sampling performed during data collection. For instance, the probability of sampling a point in a particular cell does not only depend on the total number of points in that cell, but also on which user they belong to. If all users in a cell have exactly one point in $D$, then all the points in that cell will be preserved and thus the number of points in that cell in $D_s$ will be the same as number of points in the corresponding cell in $D$. However, if users in a cell have more than ${k}$ points, then the number of points in the cell in $D_s$ is less than $D$. Due to differential privacy, information about the number of points per user in a cell can only be known by spending privacy budget, which is undesirable. 

\begin{algorithm}[t]
\begin{algorithmic}[1]
\Require A set of noisy 2-dimensional histograms, $\bar{H}$
\Ensure A set of denoised 2-dimensional histogram, $\hat{H}$
\State $\bar{T}\leftarrow \bar{H}$\label{alg:denoise:create_train}
\For{$j\leftarrow2$ to $r$}
    \For{$\bar{H}_i$ in $\bar{H}$}
        \State $\bar{H}_i^j\leftarrow$ Histogram from aggregating $j\times j$ blocks of $\bar{H}_i$ 
        \State $\bar{T}\leftarrow \bar{T}\cup\bar{H}_i^j$\label{alg:denoise:augment}
    \EndFor
\EndFor
\State {\tt encoder($.;\theta_e$)$\leftarrow$} CNN encoder with params. $\theta_e$\label{alg:denoise:enc}
\State {\tt decoder($.;\theta_d$)$\leftarrow$} TransposedCNN decoder with params. $\theta_d$ \label{alg:denoise:dec}
%\State AE($X;\theta$)$\leftarrow$ decoder(encoder($x$)), where $\theta=\theta_e\cup\theta_d$ \label{alg:denoise:ae}
\Repeat\label{alg:denoise:train_begin}
    \State $z\leftarrow$ {\tt encoder($\bar{T};\theta_e$)}\label{alg:denoise:encode}%\Comment{obtaining $\alpha$-dimensional encodings}
    \State $\hat{T}\leftarrow$ {\tt decoder($z;\theta_d$)}\label{alg:denoise:decode}
    \State $\mathcal{L}_C(\hat{T})\leftarrow \sum_i\lVert \bar{T}_i-\hat{T}_i\rVert^2$ \label{alg:denoise:reconstruction_loss}%\Comment{Reconstruction loss}
    \State $\mathcal{L}_G(z)\leftarrow d(z, \Upsilon)$\label{alg:denoise:regularization_loss}%\Comment{Regularization loss}
    \State $\mathcal{L}\leftarrow \alpha\times\mathcal{L}_G(z)+\mathcal{L}_C(\hat{T})$ \label{alg:denoise:loss}
    \State $\theta\leftarrow\theta_e\cup\theta_d$
    \State Update $\theta$ in direction $-\nabla_\theta\mathcal{L}$\label{alg:denoise:gd}
\Until{convergence}\label{alg:denoise:train_end}
\State \Return {\tt decoder(encoder($\bar{H};\theta_e)\theta_d$)}\label{alg:denoise:output}
\end{algorithmic}
\caption{Learned Denoising}\label{alg:learned_denoising}
\end{algorithm}

\subsubsection{Estimation algorithm}\label{sec:refine:alg}
Taking into account the above observations, we use mean square error minimization to decide how the answer should be scaled, which accounts for both bias and the variance, and thus ensures that if the noise is too severe it is not amplified. Moreover, rather than spending privacy budget to estimate the sampling procedure, we make simplifying assumptions to create a tractable sampling model that can be mathematically analyzed. In the remainder of this section, we first describe our sampling model and then show how mean square error minimization can be used to decide how the observed noisy answers should be scaled to accurately represent the true data.

\textbf{Notation and Modeling Assumptions}. Let $N=|D|$ be the total number of data points and $n=|D_s|$ be the observed number of data points after sampling. We make simplifying assumptions about the sampling procedure for the purpose of our analysis. Specifically, we consider the case when the $n$ points are sampled independently and uniformly at random. Let $X_i^c$ be the indicator random variable equal to 1 if the $i$-th point falls in a cell $c$. Furthermore, let $\mu_c$ be the proportion of data points in the complete dataset that are in the cell $c$, so that $N\times\mu_c$ is the total number of data points in cell $c$. We assume that the $i$-th point is sampled uniformly at random across all data points, so that $\mathds{P}(X_i^c=1)=\mu_c$. 

\textbf{Algorithm}. Our goal is to design an estimator to estimate $N\times \mu_c$ for all cells, $c$, in the histogram. Our estimator needs to be accurate, but at the same time has to preserve differential privacy. We consider the estimator $\theta_c=\gamma(\sum_iX_i^c+Lap(\frac{k}{\epsilon}))$. $\theta_c$ obtains a differentially private estimate of the observed number of points in the cell $c$ and scales it by a parameter $\gamma$. We find the parameter $\gamma$ by minimizing the mean squared error of our estimator $\theta_c$. To do so we first calculate bias and variance of our estimator.
\begin{align*}
\text{Bias}(\theta_c) &= \mathds{E}[\theta_c-N{\mu}_c]=\mu_c(\gamma n -N)\\
\text{Var}(\theta_c) &= \gamma^2(n\mu_c(1-\mu_c)+2k^2\epsilon^{-2})
\end{align*}
Thus given the mean squared error of an estimator, $\text{MSE}(\theta_c)=\text{Bias}(\theta_c)^2+\text{Var}(\theta_c)$, we obtain 
$$
\text{MSE}(\theta_c)=\gamma^2(n\mu_c(1-\mu_c)+2k^2\epsilon^{-2})+\mu_c^2(\gamma n -N)^2.
$$

Next, we find the $\gamma$ value that minimizes error across all cells. Let $m=$$\mathbb{M}$$\times$$\mathbb{M}$$\times$$\mathbb{T}$ be the number of cells in the histogram. We minimize $\sum_{c=1}^m\text{MSE}(\theta_c)$ by taking the derivative of $\sum_{c=1}^m\text{MSE}(\theta_c)$ with respect to $\gamma$ and setting it to zero. We obtain that 
\begin{align}\label{eq:gamma}
    \gamma =\frac{nNC}{2mk^2\epsilon^{-2}+(1-C)n +Cn^2}
\end{align}
minimizes $\sum_{c=1}^m\text{MSE}(\theta_c)$, where $C=\sum_{c=1}^m\mu_c^2$ is a data-dependent constant. 
It is left to determine the value of $C$, but doing so on the private data itself may require spending privacy budget. However, due to inherent properties of location datasets, in practice, $C$ can be treated as a system parameter and set---in a data-independent manner thus not consuming valuable privacy budget---to a fixed value that works. We further discuss how $C$ can be set in Sec.~\ref{sec:system:trade-offs}.







\if 0
\subsection{DP Spatial Data Release with Learned Denoising} \label{sec:spatial:algo}
Learned denoising can readily be used for spatial data release. This is shown in Alg.~\ref{alg:spatial_release}. We perform a differentially private data collection step, where a noisy histogram is obtained from the true histogram. We do this by adding DP noise to the histogram. Then, by calling Alg.~\ref{alg:learned_denoising} on the noising histogram, we obtain an accurate differentially private representation of the original histogram.


SHOULD WE PUT THE LEARNING AT MULTIPLE GRANULARITIES HERE?
Privacy accounting specifics? User level vs. event level?

\fi






==> Spatiotemporal data release (1)/related.tex <==
\noindent\textbf{Private Data Release}.
Longitudinal release of individual location updates increase risk of attack \cite{xiao2010differential, cao2017quantifying}, and requires more stringent privacy settings, e.g., user-level privacy. The work in~\cite{acs2014case} models disjoint regions of the space as separate 1-d time series. However, this limits supported query types, and cannot answer range or hotspot queries. Moreover, the granularity used is very coarse.
PrivBayes~\cite{zhang2017privbayes} is a mechanism that privately learns a Bayesian network over the data, and then returns a matrix used for fitting the parameters of the Bayes net. This can be used to then generate a synthetic dataset which can consistently answer workload queries. Budget allocation is equally split between learning the Bayesian network structure and learning its parameters. Multiplicative-Weights Exponential Mechanism (MWEM) \cite{hardt2012simple} maintains an approximating distribution over the data domain, scaled by the number of records. It updates this distribution by posing a workload of linear queries (e.g., RCQs), finding poorly answered ones, and using the multiplicative update rule to revise its estimates. AHP~\cite{zhang2014towards} seeks to group a histogram’s adjacent bins with close counts to trade for smaller noise. It utilizes LPM, and sets noisy counts below a threshold to zero. The counts are then sorted and clustered using a global clustering scheme to form a partition. SNH \cite{zeighami2022neural} uses a neural database approach to denoise the query answers, by approximating the query answers with a neural network. It requires a workload, which is not available in our setting.   


% The case of high-dimensional data was addressed by~\cite{mckenna2018optimizing, xiao2012dpcube, zhang2017privbayes}. DPCube~\cite{xiao2012dpcube} searches for dense `subcubes' of the datacube representation to release privately. A part of the privacy budget is used to obtain noisy counts using LPM over a straightforward partitioning, which is then improved to a standard kd-tree. Fresh noisy counts for the partitions are obtaining with the remaining budget and a final inference step resolves inconsistencies between the two sets of counts, and improves accuracy. Lastly, PrivBayes~\cite{zhang2017privbayes} learns a Bayesian network over the data distribution in order to generate from it a synthetic dataset which can consistently answer workload queries. Budget allocation is equally split over learning the Bayesian network structure and learning its network parameters.

\noindent\textbf{Noise reduction techniques}. 
Most deep-learning based denoising methods \cite{im2017denoising, pang2021recorrupted, lehtinen2018noise2noise} rely on many pairs of clean/noisy images. Denoising autoencoders attempt to learn original data distributions that have been corrupted according to some noise distribution, (e.g., by maximizing the log probability of the clean input, given a noisy input). Recent work in \cite{krull2019noise2void}
trains a model from noisy/noisy image pairs, by extracting noisy versions of the same image repeatedly.  Such a training process is not viable under DP since it would require additional privacy budget for each noisy extraction. Some mild noise from images can also be removed in an unsupervised fashion \cite{zheng2020unsupervised, quan2020self2self}. No approach studied denoising in the presence of DP.%, which tends to distort data significantly more.

\noindent\textbf{Privacy preserving machine learning}. 
% SNH\cite{zeighami2021neural} used Multi-Layer-Perceptrons (MLP) as universal function approximators \cite{hornik1989multilayer}. The learned function is limited to spatial range count queries. As opposed to the CNNs used in our work, SNH consumes significantly more number of parameters in its MLPs, and is only useful when the amount of training data is small or when very precise query workload is known.
A learned model may leak information about the data it was trained on \cite{shokri2017membership,hitaj2017deep}. Application of DP to empirical risk minimization \cite{chaudhuri2011differentially, kifer2012private} and deep neural networks \cite{sealfon2021efficiently, abadi2016deep} has been recently explored. Existing approaches add noise to the output of the trained model \cite{wu2017bolt}, add a random regularization term to the objective function ~\cite{chaudhuri2011differentially, kifer2012private}, or add noise to the gradient of the loss function during training~\cite{abadi2016deep}.
Our approach sanitizes the training data {\em before} learning. Furthermore, the work of \cite{abadi2016deep} achieves ($\varepsilon, \delta$)-DP~\cite{nissim2007smooth, erlingsson2014rappor, censusgovKDD18}, a weaker privacy guarantee.% than $\varepsilon$-DP which is achieved by our method.


\iffalse

A learned model can leak information about the data it was trained on \cite{shokri2017membership,hitaj2017deep}. %, 
Recent efforts have developed differentially private versions of ML algorithms, e.g., empirical risk minimization \cite{chaudhuri2011differentially, kifer2012private} and deep neural networks \cite{sealfon2021efficiently, abadi2016deep}. For DP sanitization, existing approaches add noise to the output of the trained model \cite{wu2017bolt}, add a random regularization term to the objective function ~\cite{chaudhuri2011differentially, kifer2012private}, or add noise to the gradient of the loss function during training~\cite{abadi2016deep}.
%and releases the minima of the perturbed objective, 
%and gradient perturbation algorithms, which . %Based on the familiar sensitivity method proposed by Dwork et al.\cite{dwork2008differential}, 
%Output Perturbation~\cite{wu2017bolt} perturbs the output answers after the training procedure. The variance of the added noise corresponds to the maximum distance of the output parameters for any two neighboring input datasets. 
%Objective perturbation~\cite{chaudhuri2011differentially, kifer2012private} perturbs the objective function by adding a random regularization term and releases the minima of the perturbed objective. 
%The first two approaches ensure privacy for algorithms that optimize a convex objective such as ERM, while gradient perturbation guarantees differential privacy  even for non-convex objectives, e.g., in deep neural networks. 
Our approach is different in that we sanitize the training data {\em before} learning. Furthermore, the work of \cite{abadi2016deep} achieves ($\varepsilon, \delta$)-DP~\cite{nissim2007smooth, erlingsson2014rappor, censusgovKDD18}, a weaker privacy guarantee.% than $\varepsilon$-DP which is achieved by our method.
%, is the de-facto privacy standard for data publishing.

\noindent\textbf{Private Data Release}. 
%The task of answering RCQs is well explored in the literature. Classes of algorithms can be categorized based on data dimensionality and their data-dependent or independent nature.

In the one dimensional case, the data-independent Hierarchical method \cite{hay2009boosting} uses a strategy consisting of hierarchically structured range queries typically arranged as a tree. Similar methods (e.g., HB  ~\cite{qardaji2013understanding}) differ in their approach to determining the tree's branching factor and allocating appropriate budget to each of its levels. Data-dependent techniques, on the other hand, exploit the redundancy in real-world datasets to boost the accuracy of histograms. The main idea is to first lossily compress the data. For example, EFPA \cite{acs2012differentially} applies the Discrete Fourier Transform  whereas DAWA~\cite{li2014data} uses dynamic  programming to compute the least cost partitioning. The compressed data is then sanitized, for example, directly with Laplace noise~\cite{acs2012differentially} or with a greedy algorithm that tunes the privacy budget to an expected workload~\cite{li2014data}).  

While some approaches such as DAWA and HB extend to 2D naturally, others specialize to answer spatial range queries. Uniform Grid (UG) \cite{qardaji2013differentially} partitions the domain into a $m \times m$ grid and releases a noisy count for each cell. The value of $m$ is chosen in a data-dependent way, based on dataset cardinality. Adaptive Grid (AG) \cite{qardaji2013differentially} builds a two-level hierarchy: the top-level partitioning utilizes a granularity coarser than UG. For each bucket of the top-level partition, a second partition is chosen in a data-adaptive way, using a finer granularity for regions with a larger count. QuadTree~\cite{cormode2012differentially} first generates a quadtree, and then employs the Laplace mechanism to inject noise into the point count of each node. Range-count queries are answered via a top-down traversal of the tree. Privtree \cite{zhang2016privtree} is another hierarchical method that allows variable node depth in the indexing tree (as opposed to fixed tree heights in AG, QuadTree and HB). It utilizes the Sparse-Vector Technique \cite{svtvldb2017} to determine a cell's density prior to splitting the node.


\fi

==> Spatiotemporal data release (1)/response.tex <==
\twocolumn
\noindent
\thispagestyle{empty}

\begin{comment}

\vspace{-25pt}
\section{FULL COMMENTS}

{\tt GG: this stays here just for our ease of reference and will be removed for submission, check page 3 for response letter}



\subsection{Meta-Reviewer Comments}
\begin{mrcomment}
``Provide better reasons for design choices, experiments settings and
hyperparameters tuning other than "we found that this is the best".''
\end{mrcomment}

\noindent\textbf{Response.} 


\begin{mrcomment}
``Provide better explanation for the experiments rather than giving many
many of them without detailed experiments.
''
\end{mrcomment}


\begin{mrcomment}
``Provide more clarify on assumptions on the context of the applications
(eg. set k empirically from data of which city) and on the distribution of the
data.
''
\end{mrcomment}


\subsection{Comments Reviewer 1}
\begin{comment1}
``Restore the correct spacing around captions and section headings, according to the ACM style file (i.e., remove any negative vspace, titlesec or sectsty packages etc.
''
\end{comment1}


\begin{comment1}
``Increase the size of plots to make them readable (O1)''
\end{comment1}


\begin{comment1}
``Discuss in more detail how the hyperparameters are chosen''
\end{comment1}

\subsection{Comments Reviewer 2}




\begin{comment2}
``O1 - IMPACT OF ASSUMPTIONS: A number of assumptions are made about the data which limits applicability of the proposed solution. These limitations should either be addressed or clearly explained. For example, the authors assume that “patterns (in the spatiotemporal data] are consistent and repeating over time and therefore representation learning can be achieved effectively using image feature learning”. The reviewer is not sure if the expected patterns existing in all spatiotemporal datasets. This is important as VAEs rely on existence of such common patterns and if a dataset fails to comply with this assumption it is not clear how the proposed solution would apply. On a related note, even if such patterns exist in a spatiotemporal dataset (due to some real-world continuous-time phenomenon captured by the data), the patterns may only be observed if the snapshots in the discretized data are captured at the right temporal resolution. In the paper choice of temporal resolution is ad hoc. A more rigorous analytical and empirical discussion and evaluation of the impact of temporal resolution in performance of the proposed method should be included.''
\end{comment2}


\begin{comment2}
``O2 - REMOVAL OF MEANINGFUL DATA NUANCES ALONG WITH NOISE: While VAEs are known to “denoise” the data, they might not only remove the noise introduced by the DP mechanism but the meaningful nuances in the data, affecting utility of the data for queries that are sensitive to such nuances such as spatial outlier detection queries. Performance of the proposed solutions in presence of such downstream tasks should be evaluated.''
\end{comment2}

\begin{comment2}
``O3 – VAE PARAMETERS: The ability of VAE in capturing the common patterns in the data (and as a result, denoising the data) heavily depends on whether its hyperparatmeters are tuned properly for the specific dataset on hand. In particular, depending on the size of latent space the model might either fail to capture the common patterns or capture a noisy version. It is not clear how the right parameters can be effectively determined for the proposed solution, nor impact of this is studied in the paper. On a separate but related note, the authors should clarify what they use as codebook for training VQ-VAE? Finally, multi-resolution data augmentation is proposed to generalize the model; the reviewer wonders why this is not explored by tuning the CNN used in the model, as CNN offers the same capability perhaps more rigorously.''
\end{comment2}



\subsection{Comments Reviewer 3}
\begin{comment3}
``O3: Overall, the basic idea of fixed-size samples to control noise does not seem to be effective in practice. Varying distributions across users seems hard to represent as a fixed-size sampled cloud of (x,y,t) points. Say user A has 20 trips with 20 trajectory points each, user B has 100 trips with 4 trajectory points each, and user C has 1 trip with 400 trajectory points. A,B,C have 400 points. Sampling 100 points at random from these from each of these will be a poor representation of the true distribution; there is not enough information to recover the patterns. In practice, the power law distributions we see mean that the number of points of the highest few users will be orders of magnitude more than the majority — all users with more than k points are sampled uniformly at random, which means we will lose this massive skew. (See O8 as well).''
\end{comment3}

\begin{comment3}
``O6: I appreciated the discussion of how to set k “empirically from the data of another city.” But what city? This seems interesting and could be an important contribution — there is some kind of governing process that is shared by all cities. I would have like to see more about this rather than relegating it to a kind of off-hand heuristic. Similarly, setting C to a constant warrants some more analysis: “For location datasets, we expect similar skewness across the space, and as a result, similar values of $C$ should perform well across datasets.” That’s interesting, but it needs more discussion. “Due to inherent properties of location datasets, in practice, $C$ can be treated as a system parameter and set—in a data-independent manner thus not consuming valuable privacy budget—to a fixed value that works.“ I don’t disbelieve it, but why?''
\end{comment3}


\begin{comment3}
``O12: The DP proof is in a separate technical report, but the link provided does not appear to include the proof -- the tech report looks the same as the paper? I believe it is DP since k is set as a fixed value, but there needs to be a proof. Although there appears to be no user information in the result, it still seems to be the case that the process increases the probability that a given observation in the noised histogram was contributed by a user with less than k points. In other words, we cap the heavy hitters, then scale up, which increases the contribution of the non-heavy hitters, which seems to leak information.''
\end{comment3}
\textbf{Other Comments}

[R3O7] Fig.17 compares the effects of sampling (SE) alone (no DP) to that of sampling with added DP noise (SE+NE).SE+NE lines show that without denoising,scaling at any value makes accuracy worse.Figs.18 concludes that VDR with denoising can make effective use of scaling.

\textbf{Other Comments}
[R3O9] We now have datasets CABS, GW and 4SQ in the repo.
[R3O5] The labels were inverted in Fig.14, and have been corrected. MRL markedly improves accuracy.
[R3O8] We added distributions for the mentioned datasets to Appx.of tech report (Fig.27). Power law distribution is seen for all. \textbf{Ritesh generate powerlaw for remaining geosocial datasets aswell.}
[R3O3] Codebook is designed/learned as in [55].
We add clarifying details on how VAE is trained to Sec \ref{sec:exp}



\newpage
\
\newpage
\end{comment}

\section{Response Letter}

We are grateful for the valuable feedback and suggestions. We significantly revised our original submission, all changes made are marked in \revision{\bf{blue}} color. To fit the page limit, we moved non-essential details to our anonymized technical report available online. Below are modifications (M1 -- M6) in response to required revisions.

\vspace{-10pt}
\subsection{Summary of Changes}
\noindent\textbf{M1. Data Assumptions and Their Impact on VDR}. We have added (1) a new section, Sec.~\ref{sec:data_model}, that discusses assumptions we make about the data, (2) a new paragraph in Sec.~\ref{subsec:settings} that discusses those assumptions in our datasets for our experiments and (3) a new section, Sec.~\ref{sec:assumptions_impact}, 
that summarizes where in the VDR design each of the assumptions are used and how the absence of the assumptions can potentially impact VDR. 

\textit{Density Patterns}. (Sec.~\ref{sec:data_model}:) We discuss (i) the existence of spatial and temporal patterns in the data, and (ii) why different cities are expected to have similar spatiotemporal characteristics. (i) and (ii) hold because the data is generated by urban human mobility, and similar activities (i.e., travel on the road, work commutes)  generate patterns consistent within a city and with similar characteristics across cities as observed in~\cite{yang2015nationtelescope}. We emphasize that VDR benefits from \textit{both} spatial and temporal patterns. If temporal patterns exist, VDR performance improves, but it is not essential for VDR. For example, (Sec.~\ref{subsec:settings}:) in our datasets we see temporal regularity for few locations and, in most cases, the time series at a given location is not non-stationary. This explains why, in most cases, incorporating more temporal data only marginally improves performance. Meanwhile, (Sec.~\ref{sec:assumptions_impact}:) spatial patterns are essential for VDR to denoise well and denoising ability suffers if such patterns do not exist. %(albeit marginally): up to 16 slices in Fig.~\ref{fig:learningperiod_analysis} or until 252 slices (10.5 days) in Fig.\ref{fig:transfer_learning2}. Note that first 4 points (2 days = 16 slices) of the blue (diamond marker) line in Fig.~\ref{fig:transfer_learning2} cover the same training/testing periods as in Fig.\ref{fig:transfer_learning2}, but extend it further to until 252 slices (10.5 days). In our datasets we see temporal regularity for few locations; 6.2\% (VS\_HT), 2.4\% (VS\_LA), and 1.5\% (VS\_LA) of such series exhibit non-stationarity (computation of the statistics are elaborated in Sec.\ref{subsec:settings}). In most cases, the time series at a location is *not* non-stationary. 

\textit{Power law distribution}. (Sec.~\ref{subsec:settings}:) We observed power law (PL) distribution in user contributions across all of our datasets holds (we now add the points-per-user distributions and PL function coefficients for all datasets to the Appendix~\ref{appx:data_charactaristics} of our tech report \cite{vdr_technical}, PL distribution is evidenced in all datasets)  because (Sec.~\ref{sec:data_model}:) the data is typically collected through mobile apps and user utilization across apps typically follows power law (similar to \cite{barabasi1999emergence}). (Sec.~\ref{sub:collection}:) We emphasize that \textit{due to} the power law distribution, our sampling strategy captures the bulk of density information for small values of $k$, thus lowering query sensitivity and improving the signal-to-noise ratio. However, (Sec.~\ref{sec:assumptions_impact}:) if user contributions are more uniform (e.g., all users have the same number of contributions), sampling may not be effective, and keeping all user data may achieve a better signal-to-noise ratio.


%Furthermore, Sec.~\ref{sec:assumptions_impact} discusses how  sampling may suffer if the power law distribution is not observed for a dataset. 



\noindent\textbf{M2. VAE Architecture and Hyperparameters}. We added Section~\ref{sec:dicsussion:hyperparams}, and a new experiment in Fig.~\ref{fig:gpvae_vs_vqvae}, that illustrate that (1) we chose the VAE type due to faster convergence, and different VAE types achieve similar accuracy as they all possess the required regularization ability (backed by new  Fig.~\ref{fig:gpvae_vs_vqvae}), (2) the same VAE hyperparameters, identical to \cite{razavi2019generating}, are used across all datasets and (3) the same hyperparameters perform well across all datasets due to homogeneous characteristics in location datasets (also see M1).

\noindent\textbf{M3. System Parameters, $C$ and $k$}. We added a new experiment (Fig.~\ref{fig:ulvl_growthratio}) and significantly revised the discussion in Sec.~\ref{sec:exp:ulevel:params}, regarding how we set the parameters $C$ and $k$. The new figure, Fig.~\ref{fig:ulvl_growthratio}, shows that the same value of growth ratio, $\lambda$, (which decides the parameter $k$), performs well across cities, which together with Fig.~\ref{fig:vdr_vs_debiasingC}, confirm that $C$ and $k$ can be set independent of data, due to similar density characteristics of location datasets. Finally, the new added Sec.~\ref{sec:data_model} discusses why we expect similar density characteristics across location datasets in different cities (also see M1). 


\noindent\textbf{M4. System parameters, grid granularity}. We added a new experiment (Fig.~\ref{fig:temporal_resolution}) and significantly revised the discussion in Sec.~\ref{sec:spatiotemproal_resolution} on choosing grid granularity. We suggest domain specific settings where high resolution grids are preferred to avoid otherwise using uniformity assumption to answer queries (which introduces biases). The new Fig.~\ref{fig:temporal_resolution} studies the impact of temporal resolution (i.e., time discretization), showing consistent accuracy at resolution 3h or coarser at $\varepsilon=0.4$. 

\noindent\textbf{M5. Experiments clarity}. We have rewritten almost all of Sec.~\ref{sec:exp} (only newly-added contents are marked in blue as otherwise the entire section would've been marked), answering various reviewers' questions, accommodating their suggestions and correcting typos. We have moved unnecessary figures to our technical report \cite{vdr_technical}, focused on clarity of explanation, removed the spacing overrides and made the plots larger. 

\noindent\textbf{M6. Query Limitations}. We added a paragraph to Sec.~\ref{sec:query_discussions} discussing the appropriateness of VDR in answering aggregate queries that are compatible with the objectives of differential privacy.  Queries that ask for record-level nuances (e.g., spatial outliers) or user-level information (e.g., distribution of locations per user) are not supported by VDR as they leak individual information that DP protects.


\vspace{-0.15cm}
\subsection{Response to Meta-Reviewer}
\noindent
\textbf{[MR,C1]}
{\em ``...reasons for design choices, experiments  ...''}
Addressed in M1-M4.
\noindent
\textbf{[MR,C2]} {\em  ``...explanation for the experiments...''}
% We reduced the number of plots and expanded our interpretation/discussion of results. Additional plots are included in our tech report.
Addressed in M5.
\noindent
\textbf{[MR,C3]} {\em  ``...clarify on assumptions...''}
Addressed in M1-M4.



\vspace{-0.15cm}
\subsection{Response to Reviewer 1}
\noindent
\textbf{[R1,O1]} Please see M5. 
%We have removed the spacing overrides, reduced the number of plots and expanded our interpretation/discussion of results. Additional plots are moved to our tech report.
%
\noindent\textbf{[R1,O2]} Please see M2. 
%
%We introduce a discussion on VAE model architectures (e.g., the choice of discrete vs continuous VAEs) in Sec.~\ref{sec:dicsussion:hyperparams}. We empirically compare the learning ability of the two architectures in Fig.~ \ref{fig:gpvae_vs_vqvae} and Sec.~\ref{subsec:settings}. The choice of VAE architecture is not critical, as long as they exhibit good regularization ability (as shown in Fig.~\ref{fig:regularization_analysis} in Sec.~\ref{sec:exp:comparison}).
%
\noindent\textbf{[R1,Minor Remarks]} Please see M4. The granularity in running example and synthetic data has been chosen for better visualization. 

\vspace{-0.15cm}
\subsection{Response to Reviewer 2}
\noindent\textbf{[R2,O1]}
Please see M1 regarding data assumptions and M4 regarding the impact of time discretization (grid resolution).%We add Sec.~\ref{sec:data_model} that discusses assumptions on the data and Sec.~\ref{sec:assumptions_impact} that discusses how the assumptions are used in VDR and how they impact its performance. We have added an experiment (see Fig.~\ref{fig:temporal_resolution}) in Sec.~\ref{subsec:system_modelling} that shows how temporal resolution changes accuracy. We have updated Sec.~\ref{sec:spatiotemproal_resolution} to better discuss how we set spatio-temporal resolutions and what the limits of the data release resolutions are. 
% I REMOVED THIS PARAGRAPH, WE DIDN'T KNOW WHAT THIS MEANT
%Experiments against baselines in 5.2 are entirely on 2D data (competitors cannot support inputs beyond 2D) -- hence NO temporal patterns, and we still outperform significantly.
% ITEMS LEFT: 
% Quantify the stationarity in datasets; analyze its impact on VDR performance;  and extend the range in Fig.15.
% per cell evaluate ACF, and see if seasonality exists. hopefully there are very few where seasonality exists.
% if there are many then we might need to divide error on cells with good seasonality vs not. or some grade.
\noindent \textbf{ [R2,O2]} Please see M6. %Limitation of VDR in learning data nuances is now noted in Sec.~\ref{sec:query_discussions}.
%
\noindent
\textbf{[R2,O3]} Please see M2 and M1 for hyperparameter setting. Codebook training and difference between CNNs and MRL are now clarified in Sec.~\ref{subsec:settings} and Sec.~\ref{sec:decnoising_detail}, resp. %Multi-resolution learning (MRL),as opposed to tuning CNN layers,changes the loss to explicitly enforce accurate reconstruction at multiple granularities (loss is over all training data i.e., at different granularities),which we found to provide more consistent benefits than tuning CNNs.
%
\noindent
\textbf{[R2,O4]} Please see response to R2O1 and also M1. 
%
\noindent
\textbf{[R2,O5]} Please see M3 and M1.
%We have added a new experiment (Fig.\ref{fig:gpvae_vs_vqvae} in Sec.~\ref{subsec:settings}) showing different choices, a new discussion in Sec.~\ref{sec:dicsussion:hyperparams} on how the parameters are chosen across datasets and why it is effective, which depends on the newly added discussion in Sec.~\ref{sec:data_model}. 
%
\textbf{\noindent[R2,Minor Remarks]} Please see M1 and M5. 
%
\vspace{-0.15cm}
\subsection{Response to Reviewer 3}
\noindent\textbf{[R3,O3]} Please see M1 and M6. 
%Limitations of sampling from a power-law distribution are now added to Sec.~\ref{sec:assumptions_impact} (see A1 and also response to [R3O8]). We also note the limitation on queries VDR can answer in Sec.~\ref{sec:query_discussions}.       
%
\noindent\textbf{[R3,O6]} Please see M3 and M1. 
%Using location data from a different city to set system parameters is common with DP and is justified by many studies showing that human mobility has similar characteristics across cities. We clarify these assumptions with a new discussion in Sec.~\ref{sec:data_model} and Sec.~\ref{sec:dicsussion:hyperparams}. To support our discussion w.r.t. to VDR, we add a new experiment in Fig.~\ref{fig:ulvl_growthratio} presents parameter transfer across cities. In conjunction with Fig.~\ref{fig:vdr_vs_debiasingC}, and the newly added discussion in Sec.~\ref{sec:exp:ulvl}, we show that our chosen system parameters show good accuracy on a wide array of spatial datasets with varying characteristics.
% We have more discussed these location data properties in Sec.~\ref{sec:data_model}. We have also added a new experiment (Fig.~\ref{fig:ulvl_growthratio} in Sec.~\ref{sec:exp:ulvl}) to further empirically verify this parameter transfer across cities.
%
% ITEM LEFT:
% Statistics about different power law
% Maybe add the queries the review mentions to the section where we talk about queries we don't do
%
%If similarity exists over multiple time slices, we improve performance (albeit marginally): up to 16 slices in Fig.~\ref{fig:learningperiod_analysis} or until 252 slices (10.5 days) in Fig.\ref{fig:transfer_learning2}. Note that first 4 points (2 days = 16 slices) of the blue (diamond marker) line in Fig.~\ref{fig:transfer_learning2} cover the same training/testing periods as in Fig.\ref{fig:transfer_learning2}, while the remaining of the line extends it further to until 252 slices (10.5 days). We improve performance marginally, but after the initial period improvement stagnates. These conclusions have been now drawn out in Sec~\ref{?}
%
% ITEMS LEFT:
% Change discussion in Sec.~\ref{sec:exp:ulvl} to talk about this parameter transfer
%
% Change Sec.~\ref{sec:sampling_parameters} to use Sec.~\ref{sec:data_model} when talking about parameter setting
\noindent
\textbf{[R3,O12]} As formalized in Theorem 1 of \cite{kellaris2013practical}, which we now reference in Sec.~\ref{subsec:priv_anal}, bounding user contribution ensures that prolific users appear as active as those with few check-ins, so that an adversary cannot distinguish between these two types of users. The full DP proof continues to be available in the technical report \cite{vdr_technical}.
%
%\noindent
 %We add the points-per-user distributions for all datasets to the Appendix of our tech report. In Table~\ref{tbl:table_power_law}, we report the curve fit parameters for power-law function  $f(x) = a \times x^b$ fitted to the histograms in Figs.~\ref{fig:datasets_power_law} and \ref{fig:datasets_power_law_vs}. Power law distribution is evidenced in all datasets.
\noindent
\textbf{[R3,O5]} Please see M5, M2 and M1. The labels in Fig.\ref{fig:mrl_comparison} have been corrected, MRL  improves accuracy.
%\textbf{Other Comments}
\noindent
\textbf{[R3O7]} Please see M5. \textbf{[R3O8]} Please see M1.
%Fig.~\ref{fig:NEvsSE} compares the effects of sampling (SE) alone (no DP) to that of sampling with added DP noise (SE+NE). SE+NE lines show that without denoising, scaling at any value makes accuracy worse. Figs. \ref{fig:debiasing_factor} concludes that VDR, with denoising, can make effective use of scaling. We have now made more explicit these conclusions in Sec.~\ref{subsec:ulvlchallenges}.
%
\noindent
\textbf{[R3O9]} We now have datasets CABS, GW and 4SQ in the repo.
\noindent \textbf{[R3O1]} We have revised the text.
%
\noindent \textbf{[R3O10]} Please see M4.
%
%\noindent 
\textbf{[R3O11]} Please see M6.
%
%\noindent 
\textbf{[R3O13]} Please see M2.


%\noindent
%[R3O3] Codebook is designed/learned as in  %\cite{van2017neural}.
%We expand on how VQVAE is trained in Sec.~ \ref{sec:exp:settings}


==> Spatiotemporal data release (1)/system.tex <==
\begin{algorithm}[t]
\begin{algorithmic}[1]
\Require A dataset $D$, privacy budget $\epsilon$, spatial, $\mathbb{M}$, and temporal, $\mathbb{T}$, discretization granularity, sampling parameter $k$, and refinement factor $C$. 
\Ensure Differentially private 3d-histogram $\hat{H}$ of $D$
\State $D_s\leftarrow$ sample $k$ points per user in $D$\label{alg:final:sample}
\State $H_s\leftarrow$ $\mathbb{M}$$\times$$\mathbb{M}$$\times$$\mathbb{T}$ histogram of $D_s$\label{alg:final:discritize}
\State $\bar{H}\leftarrow H_s+Lap(\frac{k}{\epsilon})$\label{alg:final:noise}
\State $\hat{H}\leftarrow \text{Denoise}(\bar{H})$\label{alg:final:denoise}
%\State $m\leftarrow$ number of cells in $\Tilde{\mathcal{H}}$
%\State $n\leftarrow$ $|D_s|$, $N\leftarrow$ $|D|$
%\State $\alpha \leftarrow\frac{nNC}{2mk^2\epsilon^{-2}+(1-C)n +Cn^2}$
\State \Return $\gamma_C\times \hat{H}$\label{alg:final:upsample}
\end{algorithmic}
\caption{\name{} algorithm}\label{alg:final_alg}
\end{algorithm}

\subsection{Privacy Analysis}\label{subsec:priv_anal}
Alg.~\ref{alg:final_alg} shows our proposed end-to-end algorithm. Lines~\ref{alg:final:sample}-\ref{alg:final:noise} correspond to the data collection step, line~\ref{alg:final:denoise} calls Alg.~\ref{alg:learned_denoising} to perform learned denoising and line~\ref{alg:final:upsample} uses the value of $\gamma_C$ calculated in Eq.~\ref{eq:gamma} to scale the results (we write it as $\gamma_C$ to make explicit the dependence on the factor $C$). Alg.~\ref{alg:final_alg} only accesses the data in the data collection step. Thus, lines~\ref{alg:final:denoise}-\ref{alg:final:upsample} can be seen as a post processing step and do not consume any privacy budget. Data collection is $\epsilon$-DP, and thus the entire \name{} provides $\varepsilon$-DP, as proved by the following:

\begin{theorem}
Algorithm~\ref{alg:final_alg} is $\epsilon$-DP.
\end{theorem}
%\textit{Proof sketch}. Data collection step is clearly $\varepsilon$-DP and the other steps of the algorithm can be seen as post-processing steps, and thus, Algorithm~\ref{alg:final_alg} is $\varepsilon$-DP. See . %HOW DO WE ACCOUNT FOR PRIVACY IN CALCULATING $\alpha$?\qed
\revision{The proof builds upon \cite{dwork2014algorithmic,kellaris2013practical} (privacy guarantee of our sampling approach follows Theorem 1 of \cite{kellaris2013practical})} and is available in our extended technical report \cite{vdr_technical}.

%We next consider system parameter setting, parameter trade-offs, and its use-case when data is released over time.

\subsection{\name{} Design Choices}\label{sec:query_discussions}
Real world use-case of spatio-temporal data extends beyond simple range count queries that are commonly studied and optimized-for in common approaches to location data release, which are typically partitioning-based \cite{qardaji2013differentially, qardaji2013differentially, zhang2018ektelo,qardaji2013understanding, zhang2017privbayes, zhang2014towards, hardt2012simple}. Other common query types such as forecasting POI visits, or finding hotspots, are sensitive to biases that such approaches introduce, causing them to perform poorly. VDR's approach of denoising a histogram created by Laplace mechanism (LPM) offers significant benefits across different spatio-temporal queries by avoiding implicit biases. 

\textbf{Forecasting Queries}. Forecasting methods are often robust to random noise present in real data, some even explicitly incorporating its effects in their models. Thus, a DP mechanism that only introduces random noise, such as LPM, can perform well, whereas those that approximate the density of regions by cleverly grouping and partitioning the domain introduce additional bias and obliterate trends and seasonal effects present in the timeseries.

\textbf{Hotspot Queries}. If a DP mechanism underestimates counts in the region of a hotspot, it will receive a distance penalty due to not having found the correct spot, and may incur a large {\em regret}, up to the maximum density threshold. This happens if an approach creates coarse partitions of the data, thus underestimating the density for `hot' peaks. Selectively creating finer partitions can improve the result, since some `hot' peaks may be preserved. Nonetheless, modelling errors in deciding where to create fine partitions can cause underestimation in some regions, resulting in large distance penalty. On the other hand, a bias-free approach such as LPM performs better since it is not affected by a systematic reduction in data utility that partitioning approaches incur. 

\textbf{Range Count Queries}. Answering larger query ranges over LPM requires aggregating more histogram cells, each contributing additional error to the answer. Therefore, VDR is specifically designed to denoise (reduce variance) of a bias-free mechanism, smoothing out the noise by exploiting the inductive bias that spatial patterns exist in location datasets. In this way, it can improve forecasts significantly by preserving timeseries specific factors and discovering hotspots that likely meet the threshold, while not sacrificing the quality of results for range count queries.

\revision{\textbf{Applicability to Other Queries}. We focus on typical spatiotemporal queries that avoid release of user-level data in order to be consistent with differential privacy objectives. Thus, our approach is specifically useful for queries that require and/or ask for patterns within the data, as regularized learning is designed to reduce noise by learning spatial patterns in the data. However, such an approach is not suitable if a query asks for data nuances as they may not be captured along with the learned patterns, or if the query asks for user specific information (e.g., distribution of locations per user), since such leakage is in conflict with differential privacy objectives.}

\subsection{System Parameter Selection}\label{sec:system:trade-offs}
We discuss the impact of system parameters $k$, $C$ and data collection granularity on the performance of the system, and provide guidelines on how they should be set in practice.

\subsubsection{Refinement Factor and Sampling Parameter}\label{sec:sampling_parameters}
Recall that in our data collection step (Alg.~\ref{alg:final_alg} line~\ref{alg:final:sample}), we sample up to $k$ points per user and in the statistical refinement step we scale our result by a factor $\gamma_C$ (Alg.~\ref{alg:final_alg} line~\ref{alg:final:upsample}), which depends on the refinement factor $C$. Both parameters, as discussed below, depend on data skewness as well as distribution of user contributions. However, due to DP, measuring data dependent properties requires spending privacy budget, which is scarce. 
%Thus, we have avoided jointly the parameters, and we consider them as two system parameters that we independently set. Here, 
Next, we discuss potential trade-offs in the values of these system parameters, and heuristics to set each.

\textbf{Sampling parameter, $k$.} For accuracy, the sampled dataset should retain density characteristics of the original dataset. After scaling with our statistical refinement step, the obtained query answers should be close to original counts. In our real-world datasets, the true data size, $N$, plays an important role in the interplay between true data characteristics and sampled ones. Specifically, when $N$ increases, most cells in the true 3-d histogram, $H$, remain empty or retain small values, due to data sparsity, while the number of reported locations in dense cells increases. This results in a more skewed true dataset. Thus, for the sampled dataset $D_s$ to capture this skewness, we need a larger number of samples, or otherwise our estimation will have a very large variance. We conclude that the value of $k$ should grow with data size. Our experiments in Section~\ref{sec:exp:systemanalysis} corroborate this heuristic, showing that the growth ratio $\lambda$, defined as $\frac{k^*}{N}$,
where $k^*$ is the best possible sampling rate, stays almost constant across datasets of various sizes \revision{(see Fig.~\ref{fig:ulvl_growthratio})}. In fact, we observe that this value remains constant across different cities, suggesting that due to similarity in density patterns   inherent to location datasets \revision{(as discussed in Sec.~\ref{sec:data_model})}, we can set the value of $k$ to be a constant fraction of $N$. Details of these observations are presented in Sec.~\ref{sec:exp:ulvl}.

\textbf{Refinement Factor, $C$.} Recall that $C$ determines how query answers are scaled to obtain the final histogram. Our theoretical model suggests that $C=\sum_c \mu_c^2$, but we do not have access to $\mu_c$ due to differential privacy, thus we treat $C$ as a system parameter. Note that, $C$ depends on data distribution. For instance, if the data are uniformly distributed, $\mu_c$ will be equal to $\frac{N/m}{N}=\frac{1}{m}$, so that $\sum_c \mu_c^2=m\times\frac{1}{m^2}=\frac{1}{m}$. On the other hand, if all the $N$ points are in a single cell, then $\sum_c \mu_c^2=1$. For location datasets, we expect similar density patterns across the space \revision{(as discussed in Sec.~\ref{sec:data_model})}, and as a result, similar values of $C$ should perform well across datasets. Our results in Sec.~\ref{sec:exp:ulvl} confirm that the same value of $C$ can be used with distinct datasets and sampling rates \revision{(see Fig.~\ref{fig:vdr_vs_debiasingC})}. We suggest setting the value of $C$ to one that performs well on a public dataset. Having $C$ as a system parameter is advantageous because it allows for correction of errors that have been introduced due to our theoretical modeling. For instance, our analysis in Sec.~\ref{sec:refine:alg} does not take into account the impact of denoising, which we expect to be consistent across datasets. By setting $C$ as a system parameter, we can avoid any adverse impacts of modeling errors in practice. Moreover, since the modelling error is consistent across datasets, the same value of $C$ can be set for all datasets.%, and we may set the value of $C$ data independently.

%, and thus one expects the theoretical results to applicable to the case when we do not perform any denoising, that is, if we omit the denoising step in Alg.~\ref{alg:final_alg}. Nonetheless, in the absence of denoising, given the amount of sparsity in the data (i.e., most histogram cells in the true data are either zero or have very few values), any amount of scaling can adversely affect the quality of the histogram. This is because, even though scaling can help improve the accuracy for dense cells, it disproportionately makes the accuracy of sparse cells worse (see Sec.~\ref{sec:exp:ulvl} for empirical confirmation). Nonetheless, denoising reduces the magnitude of the noise, allowing scaling of the results. . Based on the definition in Sec.~\ref{sec:refine:alg}, $C=\sum_c \mu_c^2$ can be seen as a measure of skewness. 
% \vspace{-3mm}
\subsubsection{\revision{Spatio-temporal Resolution}}\label{sec:spatiotemproal_resolution}
\revision{We assume throughout our discussion that a 3-d histogram of a predefined resolution is required, which is often the case since the choice of resolution is domain specific. High-resolution density maps are preferred for location datasets in industrial data release projects~\cite{dataforgood, aktay2020google}. VDR uses a 30m$\times$30m grid and 3h temporal resolution. A coarser discretization induces partitioning biases in query answers: the answer to finer queries are estimated from the answer to their enclosing coarse cell assuming uniformly distributed points within the spatial extent (Sec.~\ref{sec:query_discussions} discusses the adverse effects of such a bias). %This has been typically challenging since publicly available location datasets are small, and thus not suitable for studying at high resolution.
%Here we discuss vaious considerations that go into choosing the granularity.
%As a result the publishing for such data has been limited to the industry. In academia, a 
 %Choice of spatial resolution has been studied before \cite{qardaji2013differentially}, where the primary concern is that 
Nonetheless, there are limits to how high the resolution of the data release can be for two reasons: (1) A fine-grained histogram will have small true count values per cell, and since scale of DP-added noise is proportional to sensitivity and not the counts, the resulting signal-to-noise ratio will be low, compromising accuracy. 
(2) The spatio-temporal resolution needs to pick up the existence of consistent spatial patterns. VDR's accuracy may suffer if too fine of a granularity is chosen, as no consistent spatial patterns may exist for the CNN layers to learn. 
We experimentally support these conjectures in Fig. \ref{fig:temporal_resolution} in Sec.~\ref{subsec:system_modelling}.}


\subsection{Impact of Assumptions}\label{sec:assumptions_impact}

%SEP: NOT SURE IF WE NEED THIS, OR IF THERE IS ANYTHING MORE INTERESTING TO SAY, BUT I MOSTLY JUST WANTED TO SUMMARIZE THE ASSUMPTIONS WE MAKE AND WHICH PART OF VDR USES THEM

\revision{Specific assumptions on spatial-data distribution (as discussed in Sec~\ref{sec:data_model}) have moulded VDR design (as discussed in \ref{sec:query_discussions}). Consequently, a discussion is warranted on the effect on VDR when these assumptions do not hold:
%characteristics in location datasets in Sec. X, which we have empriically verified to be true in real-world location dataset, and are consistent with existing understanding of urban human mobility [XX]. Here, we summarize where these data charactaristics have been used in VDR, 
%Next, we discuss and what the impact would be if VDR is to be used in a domain where such charactaristics do not exist. 
(1) The use of {\em CNNs} is predicated on the existence of repeating {\em spatial} patterns within a city. If such an assumption does not hold, model accuracy suffers. For instance, as data become more uniformly distributed, the accuracy gain of VDR compared to benchmarks is lost. However, in practice, location data are often skewed, and the release of uniform-like data is a far less challenging/interesting problem for which simpler solutions may suffice.
%In practice, Nonetheless, as the goal of releasing the data is often to utilize the existing patterns for decision making, releasing such uniorm-like data with no pattern may of less practical interest. 
(2) To avoid data-dependent parameter tuning, VDR relies on the existence of similar density patterns {\em across} cities. If this assumption fails (e.g., when considering the release of generic 3-d dataset) one may need to spend additional privacy budget on system and hyper-parameter tuning, hence overall accuracy will decrease. (3) Due to the power law distribution discussed in Sec.~\ref{sec:data_model}, our sampling strategy captures the bulk of density information for small values of $k$, thus lowering query sensitivity and improving the signal-to-noise ratio (also see Sec.~\ref{sub:collection}). However, if user contributions are more uniform (e.g., all users have the same number of contributions), sampling (or the subsequent refinement) may not be effective, and keeping all user data may acheive a better signal-to-noise ratio.}%, and incrementing it further to get more location signals of few heavy hitters only marginally adds to accuracy. Meanwhile, more data contributions per user (>> k) increases query sensitivity and requires more added noise. However, if the user contributions are more uniform, sampling (or subsequent refinement) may not be effective, as keeping all user data will only improve signal-to-noise ratio}

% the {\em power law distribution} of user contributions in location datasets enables our sampling strategy to be especially effective, since taking a few samples per user can capture the density patterns and  and our sampling (and statistical refinement) method can be effectively used in any such setting. In the case of location datasets, we bound user contributions in Sec.~\ref{sub:collection}, and , doesn't require keeping all user data to learning meaningful density patterns. Nonetheless, the applicability of sampling isn't only limited to such power law distributions.  }

%(3) The assumption onis used in our sampling strategy. By sampling only a few points per user, we can obtain enough meaningful data (see Sec.~\ref{??}). VDR only requires being able to capture meaningful data through few samples per user, which holds when user data follow the power law distribution, and can be effectively utilized when that assumption is true, irrespective of whether the original distribution is power law or not. 


\vspace{-2mm}
\subsection{Data Release over Time} So far we have considered the release of a static dataset $D$. In practice, spatiotemporal data is released over time, with new data coming in continuously. In such a setting, privacy budget is often allocated per time period, e.g., a budget of $\varepsilon_i$ would be allocated for the $i$-th week ($\varepsilon_i$ is typical set to go to zero so that $\sum_i\varepsilon_i$ is bounded). Thus, the release consists of a sequence of datasets $D_1, D_2, ...$, where each $D_i$ covers a fixed period of time. Let  $\tau$ denote the duration covered by each $D_i$, which we call release duration. To use \name{} in this setting, Alg.~\ref{alg:final_alg}, can be called for every release, where in the $i$-th release, the input dataset is $D_i$ and privacy budget is $\epsilon_i$. However, an important characteristic of \name{} is that the model does not need to be retrained for every data release. That is, rather than retraining the model in the learned denoising step for every release, after the model is trained once, it is still able to denoise the input histograms. We verify this empirically in our experiments. This also shows that our model is learning recurring patterns from data, which generalize well to unseen data points.









==> Spatiotemporal data release (1)/vdr.tex <==
%Given a dataset of location reports over time, we perform a careful sanitization process to create a DP-compliant spatio-temporal histogram. Any number of computations performed on the histogram after it is sanitized with DP are considered safe. The histogram may be thus publicly released and used to answer arbitrary downstream queries such as the ones discussed in Sec~\ref{sec:bck}. Our approach takes advantage of specific characteristics of spatio-temporal datasets to provide a customized mechanism that achieves DP. 
%We first provide an overview of our approach, and then present each step of the process in detail.

\if 0
\begin{figure}
    \centering
    \includesvg[width=\columnwidth]{illustrations/overview.svg}
    \caption{Overview}
    \label{fig:overview}
\end{figure}
\fi


%\vspace{-10pt}

\if {0}{
%\subsection{\name{} Overview}
Our approach consists of three steps: (1) {\em data collection},
%creates a noisy
%histogram of the data using the Laplace mechanism and a sampling technique that reduces %sensitivity by bounding the amount of location reports from each individual; 
(2) {\em learned denoising} 
%executes a post-processing algorithm that makes use of machine learning, specifically variational auto-encoders, to improve data accuracy; 
and (3) {\em statistical refinement}.
%uses a statistical estimator to improve query accuracy by off-setting the impact of sampling. 
We provide technical descriptions of each step in Sections~\ref{sub:collection}~-~\ref{sub:refinement}. %\revision{In Section~\ref{sub:assumptions}, we discuss our assumptions and design rationale}.
}\fi
\begin{comment}
%GG: I REMOVE THE THREE PARAGRAPHS BELOW, SINCE THEY ARE REPETITIVE COMPARED TO 3.2-3.4}

\textbf{Data Collection}
creates a noisy DP-compliant
histogram of the data using the Laplace mechanism and a sampling technique that reduces sensitivity by bounding the amount of location reports from each individual.
%combines a sampling step to the addition of noise from the Laplace mechanism to create a differentially private histogram of the dataset, without 
It makes no assumptions on the data distribution, and simply
%This results in a noisy dataset histogram. 
adds i.i.d random noise to each cell, with no modeling bias being introduced in the query answers to histogram cells. 
%By specifically considering the characteristics of spatiotemporal data, the trade-off between sampling and increased noise due to sensitivity is managed to create as accurate a histogram as possible.

\textbf{Learned Denoising} 
%The data collection step yields a noisy 3-dimensional histogram. 
learns a model that captures the spatio-temporal density patterns of the original data from the noisy histogram. Using these patterns, denoising is able to construct a histogram that answers queries more accurately. %the original data than the noisy histogram. 
It acts as a post-processing algorithm, hence the the DP requirement is preserved, and it makes use of variational auto-encoders to offset some of the excessive noise introduced by the Laplace mechanism.

\textbf{Statistical Refinement} 
scales the denoised histogram according to a DP-compliant statistical estimator to offset the effect of sampling used to decrease sensitivity during data collection.

\end{comment}

%\subsection{Design for Spatiotemporal Data Release}
%\subsubsection{Sampling and Up-sampling for User-Level Privacy}. 

%\subsubsection{Learned Denoising using Spatiotemporal Patterns}. 



%Differential privacy requires adding noise to the histogram when publishing it. To provide good utility, we need to devise a method to combat the DP noise. The traditional method to do so has been uniformity assumption, where parts of the space are aggregated and the data points in them are assumed to be uniformly distributed. Such uniformity assumptions do not hold in practice and more so in the case of spatiotemporal data, as the hide the spatiotemporal patterns through uniformity assumption. Instead, we utilize spatiotemporal patterns in the data for denoising. As shown in Fig.~\ref{fig:histogram_overtime}, spatiotemporal patterns exist in location datasets. For instance, specific pattern can be seen for data on the roads as well as various gathering areas in the city. Furthermore, the spatial patterns remain consistent over time as shown in the figure. We propose to learn a model that can capture the spatiotemproal patterns in the data without being affected by the noise. 

==> response.tex <==
\twocolumn
\noindent
\thispagestyle{empty}

\begin{comment}

\vspace{-25pt}
\section{FULL COMMENTS}

{\tt GG: this stays here just for our ease of reference and will be removed for submission, check page 3 for response letter}



\subsection{Meta-Reviewer Comments}
\begin{mrcomment}
``Provide better reasons for design choices, experiments settings and
hyperparameters tuning other than "we found that this is the best".''
\end{mrcomment}

\noindent\textbf{Response.} 


\begin{mrcomment}
``Provide better explanation for the experiments rather than giving many
many of them without detailed experiments.
''
\end{mrcomment}


\begin{mrcomment}
``Provide more clarify on assumptions on the context of the applications
(eg. set k empirically from data of which city) and on the distribution of the
data.
''
\end{mrcomment}


\subsection{Comments Reviewer 1}
\begin{comment1}
``Restore the correct spacing around captions and section headings, according to the ACM style file (i.e., remove any negative vspace, titlesec or sectsty packages etc.
''
\end{comment1}


\begin{comment1}
``Increase the size of plots to make them readable (O1)''
\end{comment1}


\begin{comment1}
``Discuss in more detail how the hyperparameters are chosen''
\end{comment1}

\subsection{Comments Reviewer 2}




\begin{comment2}
``O1 - IMPACT OF ASSUMPTIONS: A number of assumptions are made about the data which limits applicability of the proposed solution. These limitations should either be addressed or clearly explained. For example, the authors assume that “patterns (in the spatiotemporal data] are consistent and repeating over time and therefore representation learning can be achieved effectively using image feature learning”. The reviewer is not sure if the expected patterns existing in all spatiotemporal datasets. This is important as VAEs rely on existence of such common patterns and if a dataset fails to comply with this assumption it is not clear how the proposed solution would apply. On a related note, even if such patterns exist in a spatiotemporal dataset (due to some real-world continuous-time phenomenon captured by the data), the patterns may only be observed if the snapshots in the discretized data are captured at the right temporal resolution. In the paper choice of temporal resolution is ad hoc. A more rigorous analytical and empirical discussion and evaluation of the impact of temporal resolution in performance of the proposed method should be included.''
\end{comment2}


\begin{comment2}
``O2 - REMOVAL OF MEANINGFUL DATA NUANCES ALONG WITH NOISE: While VAEs are known to “denoise” the data, they might not only remove the noise introduced by the DP mechanism but the meaningful nuances in the data, affecting utility of the data for queries that are sensitive to such nuances such as spatial outlier detection queries. Performance of the proposed solutions in presence of such downstream tasks should be evaluated.''
\end{comment2}

\begin{comment2}
``O3 – VAE PARAMETERS: The ability of VAE in capturing the common patterns in the data (and as a result, denoising the data) heavily depends on whether its hyperparatmeters are tuned properly for the specific dataset on hand. In particular, depending on the size of latent space the model might either fail to capture the common patterns or capture a noisy version. It is not clear how the right parameters can be effectively determined for the proposed solution, nor impact of this is studied in the paper. On a separate but related note, the authors should clarify what they use as codebook for training VQ-VAE? Finally, multi-resolution data augmentation is proposed to generalize the model; the reviewer wonders why this is not explored by tuning the CNN used in the model, as CNN offers the same capability perhaps more rigorously.''
\end{comment2}



\subsection{Comments Reviewer 3}
\begin{comment3}
``O3: Overall, the basic idea of fixed-size samples to control noise does not seem to be effective in practice. Varying distributions across users seems hard to represent as a fixed-size sampled cloud of (x,y,t) points. Say user A has 20 trips with 20 trajectory points each, user B has 100 trips with 4 trajectory points each, and user C has 1 trip with 400 trajectory points. A,B,C have 400 points. Sampling 100 points at random from these from each of these will be a poor representation of the true distribution; there is not enough information to recover the patterns. In practice, the power law distributions we see mean that the number of points of the highest few users will be orders of magnitude more than the majority — all users with more than k points are sampled uniformly at random, which means we will lose this massive skew. (See O8 as well).''
\end{comment3}

\begin{comment3}
``O6: I appreciated the discussion of how to set k “empirically from the data of another city.” But what city? This seems interesting and could be an important contribution — there is some kind of governing process that is shared by all cities. I would have like to see more about this rather than relegating it to a kind of off-hand heuristic. Similarly, setting C to a constant warrants some more analysis: “For location datasets, we expect similar skewness across the space, and as a result, similar values of $C$ should perform well across datasets.” That’s interesting, but it needs more discussion. “Due to inherent properties of location datasets, in practice, $C$ can be treated as a system parameter and set—in a data-independent manner thus not consuming valuable privacy budget—to a fixed value that works.“ I don’t disbelieve it, but why?''
\end{comment3}


\begin{comment3}
``O12: The DP proof is in a separate technical report, but the link provided does not appear to include the proof -- the tech report looks the same as the paper? I believe it is DP since k is set as a fixed value, but there needs to be a proof. Although there appears to be no user information in the result, it still seems to be the case that the process increases the probability that a given observation in the noised histogram was contributed by a user with less than k points. In other words, we cap the heavy hitters, then scale up, which increases the contribution of the non-heavy hitters, which seems to leak information.''
\end{comment3}
\textbf{Other Comments}

[R3O7] Fig.17 compares the effects of sampling (SE) alone (no DP) to that of sampling with added DP noise (SE+NE).SE+NE lines show that without denoising,scaling at any value makes accuracy worse.Figs.18 concludes that VDR with denoising can make effective use of scaling.

\textbf{Other Comments}
[R3O9] We now have datasets CABS, GW and 4SQ in the repo.
[R3O5] The labels were inverted in Fig.14, and have been corrected. MRL markedly improves accuracy.
[R3O8] We added distributions for the mentioned datasets to Appx.of tech report (Fig.27). Power law distribution is seen for all. \textbf{Ritesh generate powerlaw for remaining geosocial datasets aswell.}
[R3O3] Codebook is designed/learned as in [55].
We add clarifying details on how VAE is trained to Sec \ref{sec:exp}



\newpage
\
\newpage
\end{comment}

\section{Response Letter}

We are grateful for the valuable feedback and suggestions. We significantly revised our original submission, all changes made are marked in \revision{\bf{blue}} color. To fit the page limit, we moved non-essential details to our anonymized technical report available online. Below are modifications (M1 -- M6) in response to required revisions.

\vspace{-10pt}
\subsection{Summary of Changes}
\noindent\textbf{M1. Data Assumptions and Their Impact on VDR}. We have added (1) a new section, Sec.~\ref{sec:data_model}, that discusses assumptions we make about the data, (2) a new paragraph in Sec.~\ref{subsec:settings} that discusses those assumptions in our datasets for our experiments and (3) a new section, Sec.~\ref{sec:assumptions_impact}, 
that summarizes where in the VDR design each of the assumptions are used and how the absence of the assumptions can potentially impact VDR. 

\textit{Density Patterns}. (Sec.~\ref{sec:data_model}:) We discuss (i) the existence of spatial and temporal patterns in the data, and (ii) why different cities are expected to have similar spatiotemporal characteristics. (i) and (ii) hold because the data is generated by urban human mobility, and similar activities (i.e., travel on the road, work commutes)  generate patterns consistent within a city and with similar characteristics across cities as observed in~\cite{yang2015nationtelescope}. We emphasize that VDR benefits from \textit{both} spatial and temporal patterns. If temporal patterns exist, VDR performance improves, but it is not essential for VDR. For example, (Sec.~\ref{subsec:settings}:) in our datasets we see temporal regularity for few locations and, in most cases, the time series at a given location is not non-stationary. This explains why, in most cases, incorporating more temporal data only marginally improves performance. Meanwhile, (Sec.~\ref{sec:assumptions_impact}:) spatial patterns are essential for VDR to denoise well and denoising ability suffers if such patterns do not exist. %(albeit marginally): up to 16 slices in Fig.~\ref{fig:learningperiod_analysis} or until 252 slices (10.5 days) in Fig.\ref{fig:transfer_learning2}. Note that first 4 points (2 days = 16 slices) of the blue (diamond marker) line in Fig.~\ref{fig:transfer_learning2} cover the same training/testing periods as in Fig.\ref{fig:transfer_learning2}, but extend it further to until 252 slices (10.5 days). In our datasets we see temporal regularity for few locations; 6.2\% (VS\_HT), 2.4\% (VS\_LA), and 1.5\% (VS\_LA) of such series exhibit non-stationarity (computation of the statistics are elaborated in Sec.\ref{subsec:settings}). In most cases, the time series at a location is *not* non-stationary. 

\textit{Power law distribution}. (Sec.~\ref{subsec:settings}:) We observed power law (PL) distribution in user contributions across all of our datasets holds (we now add the points-per-user distributions and PL function coefficients for all datasets to the Appendix~\ref{appx:data_charactaristics} of our tech report \cite{vdr_technical}, PL distribution is evidenced in all datasets)  because (Sec.~\ref{sec:data_model}:) the data is typically collected through mobile apps and user utilization across apps typically follows power law (similar to \cite{barabasi1999emergence}). (Sec.~\ref{sub:collection}:) We emphasize that \textit{due to} the power law distribution, our sampling strategy captures the bulk of density information for small values of $k$, thus lowering query sensitivity and improving the signal-to-noise ratio. However, (Sec.~\ref{sec:assumptions_impact}:) if user contributions are more uniform (e.g., all users have the same number of contributions), sampling may not be effective, and keeping all user data may achieve a better signal-to-noise ratio.


%Furthermore, Sec.~\ref{sec:assumptions_impact} discusses how  sampling may suffer if the power law distribution is not observed for a dataset. 



\noindent\textbf{M2. VAE Architecture and Hyperparameters}. We added Section~\ref{sec:dicsussion:hyperparams}, and a new experiment in Fig.~\ref{fig:gpvae_vs_vqvae}, that illustrate that (1) we chose the VAE type due to faster convergence, and different VAE types achieve similar accuracy as they all possess the required regularization ability (backed by new  Fig.~\ref{fig:gpvae_vs_vqvae}), (2) the same VAE hyperparameters, identical to \cite{razavi2019generating}, are used across all datasets and (3) the same hyperparameters perform well across all datasets due to homogeneous characteristics in location datasets (also see M1).

\noindent\textbf{M3. System Parameters, $C$ and $k$}. We added a new experiment (Fig.~\ref{fig:ulvl_growthratio}) and significantly revised the discussion in Sec.~\ref{sec:exp:ulevel:params}, regarding how we set the parameters $C$ and $k$. The new figure, Fig.~\ref{fig:ulvl_growthratio}, shows that the same value of growth ratio, $\lambda$, (which decides the parameter $k$), performs well across cities, which together with Fig.~\ref{fig:vdr_vs_debiasingC}, confirm that $C$ and $k$ can be set independent of data, due to similar density characteristics of location datasets. Finally, the new added Sec.~\ref{sec:data_model} discusses why we expect similar density characteristics across location datasets in different cities (also see M1). 


\noindent\textbf{M4. System parameters, grid granularity}. We added a new experiment (Fig.~\ref{fig:temporal_resolution}) and significantly revised the discussion in Sec.~\ref{sec:spatiotemproal_resolution} on choosing grid granularity. We suggest domain specific settings where high resolution grids are preferred to avoid otherwise using uniformity assumption to answer queries (which introduces biases). The new Fig.~\ref{fig:temporal_resolution} studies the impact of temporal resolution (i.e., time discretization), showing consistent accuracy at resolution 3h or coarser at $\varepsilon=0.4$. 

\noindent\textbf{M5. Experiments clarity}. We have rewritten almost all of Sec.~\ref{sec:exp} (only newly-added contents are marked in blue as otherwise the entire section would've been marked), answering various reviewers' questions, accommodating their suggestions and correcting typos. We have moved unnecessary figures to our technical report \cite{vdr_technical}, focused on clarity of explanation, removed the spacing overrides and made the plots larger. 

\noindent\textbf{M6. Query Limitations}. We added a paragraph to Sec.~\ref{sec:query_discussions} discussing the appropriateness of VDR in answering aggregate queries that are compatible with the objectives of differential privacy.  Queries that ask for record-level nuances (e.g., spatial outliers) or user-level information (e.g., distribution of locations per user) are not supported by VDR as they leak individual information that DP protects.


\vspace{-0.15cm}
\subsection{Response to Meta-Reviewer}
\noindent
\textbf{[MR,C1]}
{\em ``...reasons for design choices, experiments  ...''}
Addressed in M1-M4.
\noindent
\textbf{[MR,C2]} {\em  ``...explanation for the experiments...''}
% We reduced the number of plots and expanded our interpretation/discussion of results. Additional plots are included in our tech report.
Addressed in M5.
\noindent
\textbf{[MR,C3]} {\em  ``...clarify on assumptions...''}
Addressed in M1-M4.



\vspace{-0.15cm}
\subsection{Response to Reviewer 1}
\noindent
\textbf{[R1,O1]} Please see M5. 
%We have removed the spacing overrides, reduced the number of plots and expanded our interpretation/discussion of results. Additional plots are moved to our tech report.
%
\noindent\textbf{[R1,O2]} Please see M2. 
%
%We introduce a discussion on VAE model architectures (e.g., the choice of discrete vs continuous VAEs) in Sec.~\ref{sec:dicsussion:hyperparams}. We empirically compare the learning ability of the two architectures in Fig.~ \ref{fig:gpvae_vs_vqvae} and Sec.~\ref{subsec:settings}. The choice of VAE architecture is not critical, as long as they exhibit good regularization ability (as shown in Fig.~\ref{fig:regularization_analysis} in Sec.~\ref{sec:exp:comparison}).
%
\noindent\textbf{[R1,Minor Remarks]} Please see M4. The granularity in running example and synthetic data has been chosen for better visualization. 

\vspace{-0.15cm}
\subsection{Response to Reviewer 2}
\noindent\textbf{[R2,O1]}
Please see M1 regarding data assumptions and M4 regarding the impact of time discretization (grid resolution).%We add Sec.~\ref{sec:data_model} that discusses assumptions on the data and Sec.~\ref{sec:assumptions_impact} that discusses how the assumptions are used in VDR and how they impact its performance. We have added an experiment (see Fig.~\ref{fig:temporal_resolution}) in Sec.~\ref{subsec:system_modelling} that shows how temporal resolution changes accuracy. We have updated Sec.~\ref{sec:spatiotemproal_resolution} to better discuss how we set spatio-temporal resolutions and what the limits of the data release resolutions are. 
% I REMOVED THIS PARAGRAPH, WE DIDN'T KNOW WHAT THIS MEANT
%Experiments against baselines in 5.2 are entirely on 2D data (competitors cannot support inputs beyond 2D) -- hence NO temporal patterns, and we still outperform significantly.
% ITEMS LEFT: 
% Quantify the stationarity in datasets; analyze its impact on VDR performance;  and extend the range in Fig.15.
% per cell evaluate ACF, and see if seasonality exists. hopefully there are very few where seasonality exists.
% if there are many then we might need to divide error on cells with good seasonality vs not. or some grade.
\noindent \textbf{ [R2,O2]} Please see M6. %Limitation of VDR in learning data nuances is now noted in Sec.~\ref{sec:query_discussions}.
%
\noindent
\textbf{[R2,O3]} Please see M2 and M1 for hyperparameter setting. Codebook training and difference between CNNs and MRL are now clarified in Sec.~\ref{subsec:settings} and Sec.~\ref{sec:decnoising_detail}, resp. %Multi-resolution learning (MRL),as opposed to tuning CNN layers,changes the loss to explicitly enforce accurate reconstruction at multiple granularities (loss is over all training data i.e., at different granularities),which we found to provide more consistent benefits than tuning CNNs.
%
\noindent
\textbf{[R2,O4]} Please see response to R2O1 and also M1. 
%
\noindent
\textbf{[R2,O5]} Please see M3 and M1.
%We have added a new experiment (Fig.\ref{fig:gpvae_vs_vqvae} in Sec.~\ref{subsec:settings}) showing different choices, a new discussion in Sec.~\ref{sec:dicsussion:hyperparams} on how the parameters are chosen across datasets and why it is effective, which depends on the newly added discussion in Sec.~\ref{sec:data_model}. 
%
\textbf{\noindent[R2,Minor Remarks]} Please see M1 and M5. 
%
\vspace{-0.15cm}
\subsection{Response to Reviewer 3}
\noindent\textbf{[R3,O3]} Please see M1 and M6. 
%Limitations of sampling from a power-law distribution are now added to Sec.~\ref{sec:assumptions_impact} (see A1 and also response to [R3O8]). We also note the limitation on queries VDR can answer in Sec.~\ref{sec:query_discussions}.       
%
\noindent\textbf{[R3,O6]} Please see M3 and M1. 
%Using location data from a different city to set system parameters is common with DP and is justified by many studies showing that human mobility has similar characteristics across cities. We clarify these assumptions with a new discussion in Sec.~\ref{sec:data_model} and Sec.~\ref{sec:dicsussion:hyperparams}. To support our discussion w.r.t. to VDR, we add a new experiment in Fig.~\ref{fig:ulvl_growthratio} presents parameter transfer across cities. In conjunction with Fig.~\ref{fig:vdr_vs_debiasingC}, and the newly added discussion in Sec.~\ref{sec:exp:ulvl}, we show that our chosen system parameters show good accuracy on a wide array of spatial datasets with varying characteristics.
% We have more discussed these location data properties in Sec.~\ref{sec:data_model}. We have also added a new experiment (Fig.~\ref{fig:ulvl_growthratio} in Sec.~\ref{sec:exp:ulvl}) to further empirically verify this parameter transfer across cities.
%
% ITEM LEFT:
% Statistics about different power law
% Maybe add the queries the review mentions to the section where we talk about queries we don't do
%
%If similarity exists over multiple time slices, we improve performance (albeit marginally): up to 16 slices in Fig.~\ref{fig:learningperiod_analysis} or until 252 slices (10.5 days) in Fig.\ref{fig:transfer_learning2}. Note that first 4 points (2 days = 16 slices) of the blue (diamond marker) line in Fig.~\ref{fig:transfer_learning2} cover the same training/testing periods as in Fig.\ref{fig:transfer_learning2}, while the remaining of the line extends it further to until 252 slices (10.5 days). We improve performance marginally, but after the initial period improvement stagnates. These conclusions have been now drawn out in Sec~\ref{?}
%
% ITEMS LEFT:
% Change discussion in Sec.~\ref{sec:exp:ulvl} to talk about this parameter transfer
%
% Change Sec.~\ref{sec:sampling_parameters} to use Sec.~\ref{sec:data_model} when talking about parameter setting
\noindent
\textbf{[R3,O12]} As formalized in Theorem 1 of \cite{kellaris2013practical}, which we now reference in Sec.~\ref{subsec:priv_anal}, bounding user contribution ensures that prolific users appear as active as those with few check-ins, so that an adversary cannot distinguish between these two types of users. The full DP proof continues to be available in the technical report \cite{vdr_technical}.
%
%\noindent
 %We add the points-per-user distributions for all datasets to the Appendix of our tech report. In Table~\ref{tbl:table_power_law}, we report the curve fit parameters for power-law function  $f(x) = a \times x^b$ fitted to the histograms in Figs.~\ref{fig:datasets_power_law} and \ref{fig:datasets_power_law_vs}. Power law distribution is evidenced in all datasets.
\noindent
\textbf{[R3,O5]} Please see M5, M2 and M1. The labels in Fig.\ref{fig:mrl_comparison} have been corrected, MRL  improves accuracy.
%\textbf{Other Comments}
\noindent
\textbf{[R3O7]} Please see M5. \textbf{[R3O8]} Please see M1.
%Fig.~\ref{fig:NEvsSE} compares the effects of sampling (SE) alone (no DP) to that of sampling with added DP noise (SE+NE). SE+NE lines show that without denoising, scaling at any value makes accuracy worse. Figs. \ref{fig:debiasing_factor} concludes that VDR, with denoising, can make effective use of scaling. We have now made more explicit these conclusions in Sec.~\ref{subsec:ulvlchallenges}.
%
\noindent
\textbf{[R3O9]} We now have datasets CABS, GW and 4SQ in the repo.
\noindent \textbf{[R3O1]} We have revised the text.
%
\noindent \textbf{[R3O10]} Please see M4.
%
%\noindent 
\textbf{[R3O11]} Please see M6.
%
%\noindent 
\textbf{[R3O13]} Please see M2.


%\noindent
%[R3O3] Codebook is designed/learned as in  %\cite{van2017neural}.
%We expand on how VQVAE is trained in Sec.~ \ref{sec:exp:settings}

